Techniques for Constructing Efficient Lock-free Data Structures

Building a library of concurrent data structures is an essential way to simplify the difficult task of developing concurrent software. Lock-free data structures, in which processes can help one another to complete operations, offer the following progress guarantee: If processes take infinitely many steps, then infinitely many operations are performed. Handcrafted lock-free data structures can be very efficient, but are notoriously difficult to implement. We introduce numerous tools that support the development of efficient lock-free data structures, and especially trees.

==> chap-bslack/paper.tex <==
\input{header.tex}

\newcommand{\indentitems}{\setlength\itemindent{1.22em}}
\newcommand{\maxslack}{overslack tree}
\newcommand{\bslack}{B-slack tree}
\newcommand{\rbslack}{relaxed \bslack}
\newcommand{\Rbslack}{Relaxed \bslack}
\newcommand{\weight}{weight}

%\clubpenalty=10000
%\widowpenalty=10000

%\newcommand{\details}[1]{\textbf{[[[Proof details for appendix.} #1\textbf{]]]}}
\newcommand{\details}[1]{}

\begin{document}

\input{abstract.tex}


\section{Introduction}

B-trees are balanced trees designed for block-based storage media.
Internal nodes contain between $b/2$ and $b$ child pointers, and one less key.
Leaves contain between $b/2$ and $b$ keys.
All leaves have the same depth, so access times are predictable.
If memory can be allocated on a per-byte basis, nodes can simply be allocated the precise amount of space they need to store their data, and no space is wasted.
However, typically, all nodes have the same, fixed capacity, and some of the capacity of nodes is wasted.
As much as 50\% of the capacity of each node is wasted in the worst case.
This is particularly problematic when data structures are being implemented in hardware, since memory allocation and reclamation schemes are often very simplistic, allowing only a single block size to be allocated (to avoid fragmentation).
Furthermore, since hardware devices must include sufficient resources to handle the worst-case, good expected behaviour is not enough to allow hardware developers to reduce the amount of memory included in their devices.
To address this problem, we introduce \textit{\bslack s}, which are a variant of B-trees with substantially better worst-case space complexity.
%
We also introduce \rbslack s, which are a variant of \bslack s that are more amenable to concurrent implementation.
%A non-blocking implementation of a \bslack\ can be obtained using the tree update template described in \cite{paper2}.
%(Details are %will be
%provided in the full version of the paper.)
%This technique is particularly efficient with small, localized updates.
%The resulting implementation will allow updates to proceed without interfering with searches, and will continue to function correctly even if processes crash.

The development of \bslack s was inspired by a collaboration with a manufacturer of internet routers, who wanted to build a concurrent router based on a tree.
In such embedded devices, storage is limited, so it is important to use it as efficiently as possible.
%Many embedded systems are also concurrent.
A suitable tree would have a simple algorithm for updates, small space complexity, fast searches, and searches that would not be blocked by concurrent updates.
Updates were expected to be
%very
infrequent.
One naive approach is to rebuild the entire tree after each update.
Keeping an old copy of the tree while rebuilding a new copy would allow searches to proceed unhindered, but this would double the space required to store the tree.

Search trees can be either node-oriented, in which each key is stored in an internal node or leaf, or leaf-oriented, in which each key is stored at a leaf and the keys of internal nodes serve only to direct a search to the appropriate leaf.
In a node-oriented B-tree, the leaves and internal nodes have different sizes (because internal nodes contain keys and pointers to children, and leaves contain only keys).
So, if only one block size can be allocated, a significant amount of space is wasted.
Moreover, deletion in a node-oriented tree sometimes requires stealing a key from a successor (or predecessor), which can be in a different part of the tree.
This is a problem for concurrent implementation, since the operation involves a large number of nodes, namely, the nodes on the path between the node and its successor.

\bslack s are leaf-oriented trees with many desirable properties.
The average degree of nodes is high, exceeding $b-2$ for trees of height at least three.
Their space complexity is better than all of their competitors. % (see Appendix~\ref{sec-competing}). %, even some that do not support deletion.
Consider a dictionary implemented by a leaf-oriented search tree, in which, along with each key, a leaf stores a pointer to associated data.
Suppose that each key and each pointer to a child or to data occupies a single word.
Then, $\frac{2b}{b-3}n$ is an upper bound on the number of words needed to store a \bslack\ with $n > b^3$ keys.
%($\bigstar$ A tighter bound appears in Appendix~\ref{sec-maxslack-to-bslack}. \trevor{also in the analysis section's summary...})
For large $b$, this tends to $2n$, which is optimal.
Section~\ref{sec-analysis} gives a more complex upper bound, which is much better when $b$ is small.
\bslack s have logarithmic height, and the number of rebalancing steps performed after a sequence of $m$ updates to a \bslack\ of size $n$ is amortized $O(\log (n+m))$ per update.
Furthermore, the number of rebalancing steps needed to rebalance the tree can be reduced to amortized \textit{constant} per update at the cost of slightly increased space complexity, as will be explained in the full version of the paper. %(see Appendix~\ref{sec-constant-rebalancing}).

The rest of this paper is organized as follows.
Section~\ref{sec-related} surveys related work.
Section~\ref{sec-bslack} introduces \bslack s and \rbslack s.
Height, average degree, space complexity and rebalancing costs of \rbslack s (and, hence, of \bslack s) are analyzed in Section~\ref{sec-analysis}.
Finally, we conclude in Section~\ref{sec-conclusion}.






\section{Related Work} \label{sec-related}

B-trees were initially proposed by Bayer and McCreight in 1970 \cite{bayer1970organization}. Insertion into a full node in a B-tree causes it to split into two nodes, each half full.
Deletion from a half-full node causes it to merge with a neighbour.
%
Arnow, Tenenbaum and Wu proposed P-trees \cite{arnow1985p}, which enjoy moderate improvements to average space complexity over B-trees, but waste 66\% of %the space of
each node in the worst case.

A number of generalizations of B-trees have been suggested that achieve much less waste if no deletions are performed.
Bayer and McCreight also proposed B*-trees in \cite{bayer1970organization}, which improve the worst-case space complexity.
At most a third of the capacity of each node in a B*-tree is wasted.
This is achieved by splitting a node only when it and one of its neighbours are both full, replacing these two nodes by three nodes.
K{\"u}spert \cite{kuspert1983} generalized B*-trees to trees where each node contains between $\lfloor \frac{bm}{m+1} \rfloor$ and $b$ pointers or keys, where $m \le b-1$ is a design parameter.
Such a tree behaves just like a B*-tree everywhere except at the leaves.
An insertion into a full leaf causes keys to be shifted among the nearest $m-1$ siblings to make room for the inserted key.
If the $m-1$ nearest siblings are also full, then these $m$ nodes are replaced by $m+1$ nodes which evenly share keys.
Large values of $m$ yield good worst-case space complexity.

Baeza-Yates and Per-\r{a}ke Larson introduced B+trees with partial expansions \cite{baeza1989performance}.
Several node sizes are used, each a multiple of the block size.
An insertion to a full node causes it to expand to the next larger node size.
With three node sizes, at most 33\% of each node can be wasted, and worst-case utilization improves with the number of block sizes used.
However, this technique simply pushes the complexity of the problem onto the memory allocator. Memory allocation is relatively simple for one block size, but it quickly becomes impractical for simple hardware to support larger numbers of block sizes.

Culik, Ottmann and Wood introduced strongly dense multiway trees (SDM-trees) \cite{culik1981dense}.
An SDM-tree is a node-oriented tree in which all leaves have the same depth, and the root contains at least two pointers.
Apart from the root, every internal node $u$ with fewer than $b$ pointers has at least one sibling.
Each sibling of $u$ has $b$ pointers if it is an internal node and $b$ keys if it is a leaf.
Insertion can be done in $O(b^3 + (\log n)^{b-2})$ time.
Deletion is not supported, but the authors mention that the insertion algorithm could be modified to obtain a deletion algorithm, and the time complexity of the resulting algorithm ``would be at most $O(n)$ and at least $O((\log n)^{b-1})$.''
Besides the long running times for each operation (and the lack of better amortized results), the insertion algorithm is very complex and involves many nodes, which makes it poorly suited for hardware implementation.
Furthermore, in a concurrent setting, an extremely large section of the tree would have to be modified atomically, which would severely limit concurrency.

Srinivasan introduced a leaf-oriented B-tree variant called an \textit{Overflow tree} \cite{Srinivasan01011991}.
For each parent of a leaf, its children are divided into one or more groups, and an overflow node is associated with each group.
The tree satisfies the B-tree properties and the additional requirement that each leaf contains at least $b-1-s$ keys, where $s \ge 2$ is a design parameter and $b$ is the maximum degree of nodes.
Inserting a key into a full leaf causes the key to be inserted into the overflow node instead; if the overflow node is full, the entire group is reorganized.
Deleting from a leaf is the same as in a B-tree unless it will cause the leaf to contain too few keys, in which case, a key is taken from the overflow node; if a key cannot be taken from the overflow node, the entire group is reorganized.
Each search must look at an overflow node.
The need to atomically modify and search two places at once makes this data structure poorly suited for concurrent implementation.

Hsuang introduced a class of node-oriented trees called \textit{H-trees} \cite{Huang:1985:HTO:3857.3858}, which are a subclass of B-trees parameterized by $\gamma$ and $\delta$.
These parameters specify a lower bound on the number of grandchildren of each internal node (that has grandchildren), and a lower bound on the number of keys contained in each leaf, respectively.
Larger values of $\delta$ and $\gamma$ yield trees that use memory more efficiently.
When $\delta$ and $\gamma$ are as large as possible, each leaf contains at least $b-3$ keys, and each internal node has zero or at least $\lfloor \frac{b^2+1}{2} \rfloor$ grandchildren.
The paper presents $O(\log n)$ insertion and deletion algorithms for node-oriented H-trees.
The algorithms are very complex and involve many cases.
H-trees have a minimum average degree of approximately $b/\sqrt{2}$ for internal nodes, which is much smaller than the $b-2$ of \bslack s (for trees of height at least three).

\textbf{[[[fix this]]]} The full version of the paper %Appendix~\ref{sec-competing}
describes families of B-trees, H-trees and Overflow trees which require significantly more space than  \bslack s.









Rosenberg and Snyder introduced \textit{compact B-trees} \cite{Rosenberg1979}, which can be constructed from a set of keys using the minimum number of nodes possible.
No compactness preserving insertion or deletion procedures are known.
The authors suggested using regular B-tree updates and periodically compacting a data structure to improve efficiency.
However, experiments in \cite{arnow1984empirical} showed that starting with a compact B-tree and adding only 1.6\% more keys using standard B-tree operations reduced storage utilization from 99\% to 67\%.




An impressive paper by Br{\"o}nnimann et~al. \cite{bronnimann2007putting} presented three ways to transform an arbitrary sequential dictionary into a more space efficient one.
One of these ways will be discussed here; of the other two, one is extremely complex and poorly suited for concurrent hardware implementation, and the other pushes the complexity onto the memory allocator.

Br{\"o}nnimann's transformation takes any sequential tree data structure and modifies it by replacing each key in the sequential data structure with a \textit{chunk}, which is a group of $b-2$, $b-1$ or $b$ keys, where $b$ is the memory block size.
All chunks in the data structure are also kept in a doubly linked list to facilitate iteration and movement of keys between chunks. % over the keys in the data structure.
For instance, a BST would be transformed into a tree in which each node has zero, one or two children, and $b-2$, $b-1$ or $b$ keys.
All keys in chunks in the left subtree of a node $u$ would be smaller than all keys in $u$'s chunk, and all keys in chunks in the right subtree of $u$ would be larger than all keys in $u$'s chunk.
A search for key $k$ behaves the same as in the sequential data structure until it reaches the only chunk that can contain $k$, and searches for $k$ within the chunk.
An insertion first searches for the appropriate chunk, then it inserts the key into this chunk.
Inserting into a full chunk requires shifting the keys of the $b$ nearest other chunks to make room.
If the $b$ closest neighboring chunks are full, then a key is taken from each, and a new node containing $b$ keys is inserted using the sequential data structure's insertion algorithm.
Deletion is similar.
\textbf{[[[this is not precise; you can't just take one key from each. you have to take $b$ consecutive keys out and put them in a new node, then distribute the remaining $b(b-1)$ keys amongst the original $b$ nodes.]]]}
Each operation in the resulting data structure runs in $O(f(n)+b^2)$ steps, where $f(n)$ is the number of steps taken by the sequential data structure to perform the same operation.

After this transformation, a B-tree with maximum degree $b$ requires $2n+O(n/b)$ words to store $n$ keys and pointers to data.
In the worst-case, each chunk wastes $2/b$ of its space, which is somewhat worse than in \bslack s.
Furthermore, supporting fast searches can introduce significant complexity to the hardware design.
A node in the transformed B-tree contains up to $b-1$ chunks, each of which occupies one block of memory.
Therefore, hardware must be able to quickly load up to $b-1$ blocks at once, or else deciding which child pointer to follow will be slow.

$\bigstar$ Insertion and deletion in a balances search tree typically involves performing one or more \textit{rebalancing steps} in order to maintain balance.
\textit{Relaxed balanced} search trees decouple rebalancing from insertion and deletion, so that rebalancing steps can be delayed or interleaved with insertions and deletions.
A brief survey of relaxed balanced search trees can be found in \cite{DBLP:journals/acta/Larsen98}.
Larsen and Fagerberg introduced \textit{relaxed B-trees} \cite{DBLP:journals/ijfcs/LarsenF96}, which are a relaxed balanced version of B-trees.
Relaxed B-trees have very simple insertion and deletion operations, and rebalancing steps can be performed (in any order) to transform a relaxed B-tree into a B-tree.
%If rebalancing is delayed and multiple insertions or deletions are performed, then nodes may violate B-tree properties by containing too few keys and pointers.
Several of the updates to \bslack s are derivative of updates to relaxed B-trees.
Larsen and Fagerberg also improved the space complexity of relaxed B-trees while the tree is out of balance \cite{JL01abtrees}, but the worst-case space complexity is no better than in B-trees.







\section{\bslack s} \label{sec-bslack}

A \bslack\ is a variant of a B-tree. %with maximum degree $b > 4$.
Each node stores its keys in sorted order, so binary search can be used to determine which child of an internal node should be visited next by a search, or whether a leaf contains a key.
Let $p_0, p_1, ..., p_m$ be the sequence of pointers contained in an internal node, and $k_1, k_2, ..., k_m$ be its sequence of keys.
For each $1 \le i \le m$, the subtree pointed to by $p_{i-1}$ contains keys strictly smaller than $k_i$, and the subtree pointed to by $p_i$ contains keys greater than \textit{or equal to} $k_i$.
We say that the \textit{degree of an internal node} is the number of non-\nil\ pointers it contains, and the \textit{degree of a leaf} is the number of keys it contains.
This unusual definition of degree simplifies our discussion.
The degree of node $v$ is denoted $deg(v)$.
If the maximum possible degree of a node is $b$, and its degree is $b-x$, then we say it contains $x$ \textit{slack}.

\noindent A \bslack\ is a leaf-oriented search tree with maximum degree $b > 4$ in which:
\begin{compactenum}[\hspace{4.1mm}\bfseries P1:]
\item every leaf has the same depth,
\label{prop-bslack-depth}
\item internal nodes contain between 2 and $b$ pointers (and one less key),%
\label{prop-bslack-internal}
\item leaves contain between 0 and $b$ keys, and
\label{prop-bslack-leaf}
\item for each internal node $u$, the total slack contained in the children of $u$ is at most $b-1$.
%\item for each internal node $u$ with children $v_1, v_2, ..., v_{|c(u)|}$,\\
%$deg(v_1)+deg(v_2)+...+deg(v_{|c(u)|}) \ge |c(u)|b-b$.
\label{prop-bslack-slack}
\end{compactenum}
P\ref{prop-bslack-slack} is the key property that distinguishes \bslack s from other variants of B-trees. %(and we derive the name Bounded-slack tree, or \bslack, from it).
%For any internal node $u$, the sum of the degrees of its children is at most $|c(u)|b$.
%If an internal node has $|c(u)|$ children, then the sum of the degrees of its children is at most $|c(u)|b$.
%Thus, P\ref{prop-bslack-slack} says that the amount of \textit{slack}, or wasted space, amongst the children of an internal node is at most $b$ (hence the name \bslack).
It limits the aggregate space wasted by a number of nodes, as opposed to limiting the space wasted by each node.
Alternatively, P\ref{prop-bslack-slack} can be thought of as a lower bound on the sum of the degrees of the children of each internal node.
Formally, for each internal node with children $v_1, v_2, ..., v_l$, $deg(v_1)+deg(v_2)+...+deg(v_l) \ge lb-(b-1) = lb-b+1$.
This interpretation is useful to show that all nodes have large subtrees.
For instance, it %, the relation above
implies that a node $u$ with two internal children must have at least $b+1$ grandchildren.
If these grandchildren are also internal nodes, we can conclude that % use the same relation at each of these grandchildren (and some arithmetic) to show that
$u$ must have at least $b^2-b+2$ great grandchildren.

A tree that satisfies P\ref{prop-bslack-depth}, and in which every node has degree $b-1$, is an example of a \bslack.
%Another example can be constructed as follows.
Another example of a \bslack\ is a tree of height two, where $b$ is even, the root has degree two, its two children have degree $b/2$ and $b/2+1$, respectively, and the grandchildren of the root are leaves with degree $b$, except for two, one in the left subtree of the root, and one in the right subtree, that each have degree one.
This tree contains the smallest number of keys of any \bslack\ of height two.






























\subsection{\Rbslack s} \label{sec-rbslack}

A relaxed balance search tree decouples updates that rebalance (or reorganize the keys of) the tree from updates that modify the set of keys stored in the tree~\cite{relaxedbalance}.
%We now define a \textit{relaxed balance} variant of \bslack s, called \textit{\rbslack s}.
The advantages of this decoupling are twofold.
First, updates to a relaxed balance version of a search tree are smaller, so a greater degree of concurrency is possible in a multithreaded setting.
Second, for some applications, it may be useful to temporarily disable rebalancing to allow a large number of updates to be performed quickly, and to gradually rebalance the tree afterwards.

A \rbslack\ is a relaxed balance version of a \bslack\ that has weakened the properties.
A \weight\ of zero or one is associated with each node.
These \weight s serve a purpose similar to the colors red and black in a red-black tree.
We define the \textit{relaxed depth} of a node to be one less than the sum of the \weight s on the path from the root to this node.
A \rbslack\ is a leaf-oriented search tree with maximum degree $b > 4$ in which:
%\noindent A \rbslack, where $b > 4$, is a leaf-oriented search tree in which:
\begin{compactenum}[\hspace{4.1mm}\bfseries P1$'$:]
\setcounter{enumi}{-1}
\item every node with \weight\ zero contains exactly two pointers,
\label{prop-rbslack-weight-zero}
\item every leaf has the same relaxed depth,
\label{prop-rbslack-depth}
\item internal nodes contain between 1 and $b$ pointers (and one less key), and%
\label{prop-rbslack-internal}
%\item leaves contain between 0 and $b$ keys
%\label{prop-bslack-leaf}
\end{compactenum}
\begin{compactenum}[\hspace{4.1mm}\bfseries P1\hspace{1.01mm}:]
\setcounter{enumi}{2}
\item leaves contain between 0 and $b$ keys
%\label{prop-rbslack-leaf}
\end{compactenum}

%, by replacing P\ref{prop-bslack-depth} with P\ref{prop-bslack-depth}$'$, replacing P\ref{prop-bslack-internal} with the property that internal nodes have between one and $b$ pointers, and eliminating P\ref{prop-bslack-slack}.
To clarify the difference between \bslack s and \rbslack s, we identify several types of \textit{violations} of the \bslack s properties that can be present in a \rbslack.
We say that a \textit{\weight\ violation} occurs at a node with \weight\ zero, a \textit{slack violation} occurs at a node that violates P\ref{prop-bslack-slack}, and a \textit{degree violation} occurs at an internal node with only one child (violating P\ref{prop-bslack-internal}).
%Note that these are violations of the \bslack\ properties, but not violations of the \rbslack\ properties.
Observe that P1 is satisfied in a \rbslack\ with no \weight\ violations.
Likewise, P2 is satisfied in a \rbslack\ with no degree violations, and P4 is satisfied in a \rbslack\ with no slack violations.
Therefore, a \rbslack\ that contains no violations is a \bslack.
%Although a \rbslack\ satisfies much weaker properties than a \bslack,
Rebalancing steps can be performed to eliminate violations, and gradually transform any \rbslack\ into a \bslack.
%Specifically, we use rebalancing updates to set all \weight s to one, and to ensure that P\ref{prop-bslack-slack} is satisfied.

































\subsection{Updates to \rbslack s}

We now describe the algorithms for inserting and deleting keys in a \rbslack s (in a way that maintains P\ref{prop-rbslack-weight-zero}$'$, P\ref{prop-rbslack-depth}$'$, P\ref{prop-rbslack-internal}$'$ and P\ref{prop-bslack-leaf}).
%
\textbf{[[[describe these as the same operations as in kim's paper]]]}
The updates for \rbslack s are shown in Figure~\ref{fig-updates}.
There, \weight s appear to the right of nodes, and shaded regions represent slack.
If $u$ is a node that is not the root, then we let $\pi(u)$ denote the parent of $u$.
Our insertion and deletion algorithms always ensure that all leaves have \weight\ one.
%After an insertion or deletion, rebalancing steps can be performed to set the \weight s of all internal nodes to one, while maintaining P\ref{prop-bslack-depth}$'$, so that P\ref{prop-bslack-depth} will be satisfied.

\begin{figure}[tbph]
\centering
\vspace{-5mm}
%\renewcommand{\arraystretch}{3}
\begin{tabular}{ | m{2cm} | >{\centering\arraybackslash} m{11cm} | }
\hline

%\vspace{7mm}
\textbf{Delete} & \includegraphics[scale=0.7]{figures/ops-delete.pdf} \\
\hline

\vspace{7mm}
\textbf{Insert} & \includegraphics[scale=0.7]{figures/ops-insert-simple.pdf} \\
\textbf{Overflow} & \includegraphics[scale=0.7]{figures/ops-overflow.pdf} \\
%\textbf{Insert-Distribute} & \includegraphics[scale=0.7]{figures/ops-insert-distribute.pdf}\\
%\textbf{Insert-Overflow} & \includegraphics[scale=0.7]{figures/ops-insert-overflow.pdf} \\
\hline

\vspace{7mm}
\textbf{Root-Zero} & \includegraphics[scale=0.7]{figures/ops-weightroot.pdf} \\
\textbf{Root-Replace} & \includegraphics[scale=0.7]{figures/ops-newroot.pdf} \\
\hline


\vspace{7mm}
\textbf{Absorb} & \includegraphics[scale=0.7]{figures/ops-Split1.pdf} \\
\textbf{Split} & \includegraphics[scale=0.7]{figures/ops-split2-v2.pdf} \\
\hline

\vspace{7mm}
\textbf{Compress} & \includegraphics[scale=0.7]{figures/ops-compress.pdf} \\
\textbf{One-Child} & \includegraphics[scale=0.7]{figures/ops-onechild.pdf} \\
\hline
\end{tabular}
\vspace{-2mm}
%\vspace{-5mm}
\caption{Updates to \bslack s (and \rbslack s).
Nodes with \weight\ zero contain exactly two pointers.
%A tag value of -1$^*$ indicates that a tag should be -1 unless the node is the root, in which case it should be zero.
}
\label{fig-updates}
\end{figure}

\textbf{Deletion.}
First, a search is performed to find the leaf $u$ where the deletion should occur.
If the leaf does not contain the key to be deleted, then the deletion terminates immediately, and the tree does not change.
If the leaf contains the key to be deleted, then the key is removed from the sequence of keys stored in that leaf. %, and the \textit{cleanup phase} begins.
%Note that deletion maintains the properties of a \rbslack.
%\trevor{can create P4 violation only}
%\trevor{if exists, call cleanup, which fixes this violation}
%In the cleanup phase, if the children of $\pi(u)$ contain more than $b$ slack in total, then a Compress update is performed at $\pi(u)$ to reduce the number of children (and, hence, the total slack shared amongst the children of $\pi(u)$) and evenly distribute keys.
%(The Compress %, Absorb and Split updates are
%update is described in detail in Section~\ref{sec-rebalancing}.)
%As we discuss in Section~\ref{sec-rebalancing}, a Compress update that affects a node $v$ and its children may cause P\ref{prop-bslack-slack} to be violated at $\pi(v)$, and at some of the children of $v$.
%Compress updates are performed until no node violates~P\ref{prop-bslack-slack}, at which point the deletion terminates.
Deleting this key may create a slack violation. % in which case rebalancing steps can be performed to eliminate this violation.

%If, after the deletion, the children of $\pi(u)$ contain more than $b$ slack, then a Compress update must be performed at $\pi(u)$ to reduce the number of children and evenly distribute keys.
%(In actuality, it does not matter whether keys are evenly distributed.
%We choose to evenly distribute them because this will also evenly distribute any slack, and hopefully, make subsequent insertions more likely to reach a node that contains some slack, so that they involve less work.)
%The Compress update will increase the slack of the grandparent of $u$ by one, so another Compress update may be necessary.

\textbf{Insertion.}
To perform an insertion, a search is first performed to find the leaf $u$ where the insertion should occur.
If $u$ contains some slack, then the key is added to the sequence of keys in $u$, and the insertion terminates.
Otherwise, $u$ cannot accommodate the new key, so Overflow is performed.
Overflow replaces $u$ by a subtree of height one consisting of an internal node with \weight\ zero, and two leaves with \weight\ one.
%Doing this naively would violate P\ref{prop-bslack-depth}$'$.
%One way to do this correctly is to replace a leaf of \weight\ one by a subtree whose root has \weight\ zero, and whose leaves have \weight\ one.
The $b$ keys stored in $u$, plus the new key, are evenly distributed between the children of the new internal node.
If $u$ was the root before the insertion, then the new internal node becomes the new root.
Otherwise, $u$'s parent $\pi(u)$ before the insertion is changed to point to the new internal node instead of $u$.
%After the insertion, P\ref{prop-bslack-internal} and P\ref{prop-bslack-leaf} are satisfied.
%Any leaves in the subtree rooted at $\pi(u)$ have the same relaxed depth after the update as they did beforehand.
After Overflow, there is a \weight\ violation at the new internal node.
%since there is a node with \weight\ zero, P\ref{prop-bslack-depth} is violated.
Additionally, since the new internal node contains $b-2$ slack, whereas $u$ contained no slack, there may be a slack violation at $\pi(u)$. %P\ref{prop-bslack-slack} may be violated at $\pi(u)$.
%Finally, rebalancing steps are performed to eliminate any violations.
%
%After this, the cleanup phase begins.
%In the cleanup phase, if the grandparent of $u$ is not the root, then it has \weight\ zero, so Absorb and Split updates are performed until no node contains \weight\ zero.
%As soon as a Absorb is performed, the zero \weight\ is eliminated.
%However, if no Absorb is performed, then Split updates are performed to push the zero \weight\ up in the tree, until it reaches the root, where it will be eliminated.
%Once no node has weight zero, Compress updates must be performed wherever any node violated P\ref{prop-bslack-slack}.
%Absorb updates cannot cause any node to violate P\ref{prop-bslack-slack}, but Split updates can cause P\ref{prop-bslack-slack} to be violated at the two child nodes.
%Since Compress updates may necessitate other Compress updates, they are performed until no node violates~P\ref{prop-bslack-slack}, at which point the insertion terminates.
%Let $p_0, ..., p_m$ and $k_0, ..., k_{m-1}$ be the pointers and keys, respectively, of $\pi(u)$.
%Pointers $p_{\lfloor b/2 \rfloor}, ..., p_m$ and keys $k_{\lfloor b/2 \rfloor+1}, ..., k_{m-1}$ are moved from $\pi(u)$ to a new node, which becomes $\pi(u)$'s right sibling under $gp$.
%Key $k_{\lfloor b/2 \rfloor}$ is then moved from $\pi(u)$ to $gp$.

Delete, Insert and Overflow maintain the properties of a \rbslack.
They will also %The same algorithms can also be used to insert and delete keys in a \bslack, and will
maintain the properties of a \bslack, provided that rebalancing steps are performed to remove any violations that are created. %after each insertion or deletion.











\subsection{Rebalancing steps} \label{sec-rebalancing}

%Every \rbslack\ can be transformed into a \bslack\ by performing a sequence of rebalancing steps.
%Observe that Insert-Overflow can increase the number of \weight s with value -1 in the tree (by one), and it is the only update that can do this.
%The \textit{Split} updates can be used to set a \weight\ value of -1 to zero, or to move it towards the root, where it will be set to zero.
There are six different rebalancing steps for \rbslack s: Root-Zero, Root-Replace, Absorb, Split, One-Child and Compress.
\textbf{[[[describe the first four as the same operations as in kim's paper]]]}
If there is a degree violation at the root, then Root-Replace is performed.
If not, but there is a weight violation at the root, Root-Zero is performed.
If there is a \weight\ violation at an internal node that is not the root, then Absorb or Split is performed.
Suppose there are no \weight\ violations.
If there is a degree violation at a node $u$ and no degree or slack violation at $\pi(u)$, then One-Child is performed.
If there is a slack violation at a node $u$ and no degree violation at $u$, then Compress is performed.
%Suppose there are no degree violations.
%If there is a slack violation at $u$, then Compress is performed.
%The first two can be performed only when there is a violation at the root and the next three can be performed only when there is a violation at a node other than the root.
Figure~\ref{fig-updates} illustrates these steps.
%We say that a \textit{\weight\ violation} occurs at a node with \weight\ zero, a \textit{slack violation} occurs at a node that violates P\ref{prop-bslack-slack}, and a \textit{degree violation} occurs at an internal node with only one child (violating P\ref{prop-bslack-internal}).
%Note that these are violations of the \bslack\ properties, but not violations of the \rbslack\ properties.
%Additionally, a \rbslack\ that contains no violations is a \bslack.
The goal of rebalancing is to eliminate all violations, while maintaining the \rbslack\ properties.

\textbf{Root-Zero.}
Root-Zero changes the \weight\ of the root from zero to one, eliminating a \weight\ violation, and incrementing the relaxed depth of every node.
If P\ref{prop-bslack-depth}$'$ held before Root-Zero, it holds afterwards.
%If every pair of leaves had the same relaxed depth before Root-Zero, this remains true afterwards.

\textbf{Root-Replace.}
Root-Replace replaces the root $r$ by its only child $u$, and sets $u$'s \weight\ to one.
This eliminates a degree violation at $r$, and any \weight\ violation at $u$.
If $u$ had \weight\ zero before Root-Replace, then the relaxed depth of every leaf is the same before and after Root-Replace.
Otherwise, the relaxed depth of every leaf is decremented by Root-Replace.
In both cases, if P\ref{prop-bslack-depth}$'$ held before Root-Replace, it holds afterwards.

\textbf{Absorb.}
Let $u$ be a non-root node with \weight\ zero.
Absorb is performed when $\pi(u)$ contains less than $b$ pointers.
In this case, the two pointers in $u$ are moved into $\pi(u)$, and $u$ is removed from the tree.
Since the pointer from $\pi(u)$ to $u$ is no longer needed once $u$ is removed, $\pi(u)$ now contains at most $b$ pointers.
The only node that was removed is $u$ and, since it had \weight\ zero, the relaxed depth of every leaf remains the same.
Thus, if P\ref{prop-bslack-depth}$'$ held before Absorb, it also holds afterwards.
%Moreover, the depth of every leaf in the subtree rooted at $u$ has now been decremented\trevor{(?include?)}.
%Moving the pointers from $u$ to $\pi(u)$ decrements the level of every leaf that was originally in the subtree rooted at $u$.
%Since $u$ had \weight\ zero, and these pointers move to a node with \weight\ one, the relaxed level of every leaf remains the same after the update. % (so the update maintains P\ref{prop-rbslack-depth}'). %allowing us to set the \weight\ of the new node to zero without violating P\ref{prop-rbslack-depth}'.
Absorb eliminates a \weight\ violation at $u$, but may create a slack violation at $\pi(u)$.

\textbf{Split.}
Let $u$ be a non-root node with \weight\ zero.
Split is performed when $\pi(u)$ contains exactly $b$ pointers.
In this case, there are too many pointers to fit in a single node.
We create a new node $v$ with \weight\ one, and evenly distribute all of the pointers and keys of $u$ and $\pi(u)$ (except for the pointer from $\pi(u)$ to $u$) between $u$ and $v$.
Now $\pi(u)$ has two children, $u$ and $v$.
The \weight\ of $u$ is set to one, and the \weight\ of $\pi(u)$ is set to zero.
As above, this does not change the relaxed depth of any leaf, so P\ref{prop-bslack-depth}$'$ still holds after Split.
Split moves a \weight\ violation from $u$ to $\pi(u)$ (closer to the root, where it can be eliminated by a Root-Zero or Root-Replace), but may create slack violations at $u$ and $v$.

\textbf{Compress.}
%Before a Compress update can be performed, 
Compress is performed when there is a slack violation at an internal node $u$, there is no degree violation at $u$, and there are no \weight\ violations at $u$ or any of its $k \ge 2$ children.
Let $c \le kb-b$ be the number of pointers or keys stored in the children of $u$.
Compress evenly distributes the pointers or keys contained in the children of $u$ amongst the first $\lceil c/b \rceil$ children of $u$, and discards the other children.
This will also eliminate any degree violations at the children of $u$ if $c > 1$.
After the update, $u$ satisfies P\ref{prop-bslack-slack}.
Compress does not change the relaxed depth of any node, so P\ref{prop-bslack-depth}$'$ still holds after.
%
Compress removes at least one child of $u$, so it increases the slack of $u$ by at least one, possibly creating a slack violation at $\pi(u)$.
(However, it decreases the total amount of slack in the tree by at least $b-1$.)
Thus, after a Compress, it may be necessary to perform another Compress at $\pi(u)$.
Furthermore, as Compress distributes keys and pointers, it may move nodes with different parents together, under the same parent.
Even if two parents initially satisfied P\ref{prop-bslack-slack} (so the children of each parent contain a total of less than $b$ slack), the children of the combined parent may contain $b$ or more slack, creating a slack violation.
Therefore, after a Compress, it may also be necessary to perform Compress at some of the children of $u$.

\textbf{One-Child.}
One-Child is performed when there is a degree violation at an internal node $u$, there are no \weight\ violations at $u$ or any of its siblings, and there is no violation of any kind at $\pi(u)$.
Let $k$ be the degree of $\pi(u)$.
Since there is no slack violation at $\pi(u)$, there are a total of $c > kb-b = b(k-1)$ pointers stored in $u$ and its siblings.
Since $u$ has only one child pointer, each of its other $k-1$ siblings must contain $b$ pointers.
One-Child evenly distributes the keys and pointers of the children of $\pi(u)$. %are evenly distributed.
One-Child does not change the relaxed depth of any node, so P\ref{prop-bslack-depth}$'$ still holds after.
One-Child eliminates a degree violation at $u$, but, like Compress, it may move children with different parents together under the same parent, possibly creating slack violations at some children of $\pi(u)$.
So, it may be necessary to perform Compress at some of the children of $\pi(u)$.

All of these updates maintain P\ref{prop-rbslack-weight-zero}$'$, P\ref{prop-bslack-internal}$'$ and P\ref{prop-bslack-leaf}.
%Since P\ref{prop-rbslack-weight-zero}$'$ holds, $\pi(u)$ contains at most $b-1$ pointers when Absorb is applied, and exactly $b$ pointers when Split is applied.
While rebalancing steps are being performed to eliminate the violation created by an insertion or deletion, there is at most one node with \weight\ zero.

%\textbf{Cleanup.} 
%We now describe the Cleanup procedure that is invoked after an insertion or deletion creates a \weight\ or slack violation.
%Cleanup first checks which rebalancing step should be performed out of Root-Zero, Compress, Absorb and Split, and then performs it.
%If the rebalancing step is Root-Zero, then the \weight\ violation is eliminated, and Cleanup terminates.
%Whenever Cleanup performs Absorb, it might have to perform Compress at the parent.
%Whenever Cleanup performs Split at a node $u$ where there is a \weight\ violation, it will have to perform Absorb, Split or Root-Zero at $\pi(u)$, and may have to perform Compress at one or both of the children after the Split.
%Whenever Cleanup performs Compress at a node $u$ where there is a slack violation, it may have to perform Compress at some of the children of $u$, and it may have to perform Root-Replace, One-Child or Compress at $\pi(u)$.
%Whenever Cleanup performs One-Child at a node $u$ where there is a degree violation, it may have to perform Compress at some of the siblings of $u$.
%There is one small complication.
%One-Child and Compress can be performed only if there is no degree violation at the upper node.
%Thus, consecutive degree violations on a path must be fixed by performing One-Child or Compress going downward from the topmost degree violation.
%Implementation details are discussed in Appendix~\ref{sec-cleanup-impl}.
%%In a sequential setting, it is straightforward to write a recursive implementation of Cleanup that requires stack space proportional to the height of the tree.
%%\trevor{make sure this is true. also, describe some techniques for concurrent implementation?}
%%\trevor{idea for sequential impl.: fix all zero weights first. then, check all children of nodes on the search path for the need to do compresses. do all downward compresses and one-childs recursively. then, search again, and continue doing this until all violations are fixed. what about upward compresses not on the search path????}
%
%%There are six different rebalancing steps: Root-Zero and Root-Replace, which modify the root, and Compress, One-Child, Absorb and Split.

We prove that a rebalancing step can be applied to any \rbslack\ that is not a \bslack. %\ will be transformed into a \bslack\ after a finite number of rebalancing steps have been performed (in any order).

\begin{lem} \label{lem-relaxed-then-rebalance}
Let $T$ be a \rbslack.
If $T$ is not a \bslack, then a rebalancing step can be performed.
\end{lem}
\begin{proof}
If $T$ is not a \bslack, it contains a \weight\ violation, a slack violation or a degree violation.
If there is \weight\ violation, then Root-Zero, Absorb or Split can be performed.
Suppose there are no \weight\ violations.
Let $u$ be the node at the smallest depth that has a slack or degree violation.
Suppose $u$ has a degree violation.
If $u$ is the root, then Root-Replace can be performed.
Otherwise, $\pi(u)$ has no violation, so One-Child can be performed.
Suppose $u$ does not have a degree violation.
Then, $u$ must have a slack violation, and Compress can be performed.
%
%If there is a slack violation at an internal node, but no degree violation at that node, then Compress can be performed.
%If there is a degree violation at an internal node, but no slack or degree violation at its parent, then One-Child can be performed.
%
%If there is a degree violation at an internal node, and a slack or degree violation at its parent, then consider the internal node $u$ with the smallest depth that has a slack violation.
%There is no slack violation at a smaller depth than $u$.
%Consider the node $v$ at the smallest depth that has a degree violation.
%If $v$ is the root, then Root-Replace can be performed.
%Otherwise, One-Child can be performed at $\pi(v)$, since there is no degree violation at $\pi(v)$.
\qed
\end{proof}

































\section{Analysis} \label{sec-analysis}

%Due to space constraints, this section merely gives an outline of results proved about \bslack s.
%In the full version of the paper, we provide %In Appendix~\ref{sec-appendix-analysis}, we provide
%a detailed analysis of \bslack s that store $n$ keys, by giving: an upper bound on the height of the tree, a lower bound on the average degree of nodes (and, hence, utilization), and an upper bound on the space complexity.
This section provides a detailed analysis of \bslack s that store $n$ keys, by giving: an upper bound on the height of the tree, a lower bound on the average degree of nodes (and, hence, utilization), and an upper bound on the space complexity.
We first give a brief outline of the proofs and results, and then provide the full details.

Arbitrary \bslack s are difficult to analyze, so we begin by studying a class of trees called $b$-\maxslack s.
A $b$-\maxslack\ has a root with degree two, and satisfies P\ref{prop-bslack-depth}, P\ref{prop-bslack-internal} and P\ref{prop-bslack-leaf}, but instead of P\ref{prop-bslack-slack}, the children of each internal node contain a total of exactly $b$ slack.
Thus, a $b$-\maxslack\ is a \rbslack, but not a \bslack.
%A $(b,k)$-\maxslack\ is a $b$-\maxslack\ with a root of degree $k$.
Consider a $b$-\maxslack\ $T$ of height $h$ that contains $n$ keys.
We prove that the total degree at depth $\delta \le h$ in $T$ is $d(\delta) = 2^{-\delta}(\alpha^{\delta}+\gamma^{\delta})$, where $\alpha = b+\sqrt{b^2-4b}$ and $\gamma = b-\sqrt{b^2-4b}$.
%For $\delta \ge 0$, $d(\delta)$ is an integer.
Since the total degree at the lowest depth is precisely the number of keys in the tree, every $b$-\maxslack\ of height $h$ contains exactly $d(h)$ keys.
%We immediately obtain the upper bound $h \le h_0$, where $h_0$ is the smallest integer that satisfies $d(h_0) \ge n$.
Furthermore, when $h \ge 3$, we also have $(b-2)^{h} < d(h) \le b^{h}$.
Therefore, for $n > b^3$ (which implies height at least three), $h$ satisfies $\lceil \log_b n \rceil \le h \le \lceil \log_{b-2} n\rceil$.
We also prove that the average degree of nodes in $T$ is $\frac{b\cdot d(h-1)-b+2}{b\cdot d(h-2)-b+3}$, which is greater than $b-2$ for $h \ge 3$.

We next prove some connections between \maxslack s and \bslack s.
First, we show that each $b$-\maxslack\ of height $h$ has a smaller total degree of nodes at each depth than any \bslack\ of height $h$.
We do this by starting with an arbitrary \bslack\ of height $h$, and repeatedly removing pointers and keys from the children of each internal node that satisfies P\ref{prop-bslack-slack} (taking care not to violate P1, P2 or P3), until we obtain a $b$-\maxslack.
It follows that each $b$-\maxslack\ of height $h$ contains fewer keys than any \bslack\ of height $h$.
Consequently, every $b$-\maxslack\ with $n$ keys has height at least as large as any \bslack\ with $n$ keys.
We next prove that every $b$-\maxslack\ of height $h$ has a smaller average node degree than any \bslack\ of height $h$.
As above, the proof starts with an arbitrary \bslack\ of height $h$, and removes pointers and keys from nodes until the tree becomes a $b$-\maxslack.
However, in this proof, every time we remove a pointer, we must additionally show that the average degree of nodes in the tree decreases.

%We then show that an \maxslack\ of height $h$ whose root has degree two has fewer keys than any \bslack\ of height $h$ (Corollary~\ref{cor-2maxslack-worst-case-height}) and a smaller average degree than any \bslack\ of height $h$ (Lemma~\ref{lem-D-lower-bound-for-bslack} and \ref{lem-2maxslack-worst-case-Dbar}).
%We use this lower bound on average degree to compute an upper bound on the space complexity of any \bslack\ with $n$ keys.

We then compute the \textit{space complexity} of a \bslack\ containing $n$ keys, which is the number of words needed to store it.
%We then use the lower bound on the average degree of nodes in a \bslack\ $T$ of height $h$ to compute the space complexity of $T$.
Consider a leaf-oriented tree with maximum degree $b$.
For simplicity, we assume that each key and each pointer to a child or data occupies one word in memory.
Thus, a leaf occupies $2b$ words, and an internal node occupies $2b-1$ words.
A memory block size of $2b$ is assumed.
Let $\bar D$ be the average degree of nodes.
Then, $U = \bar D/b$ is the proportion of space that is utilized (which we call the \textit{average space utilization} of the tree), and $1-U$ is the proportion of space that is wasted.
The space complexity is $2bF$, where $F$ is the number of nodes in the tree.
Suppose the tree contains $n$ keys.
%Let us compute its space complexity.
By definition, the sum of the degrees of all nodes is $F - 1 + n$, since each node,
except the root, has a pointer into it and the degree of a leaf is the number of keys it contains.
Additionally, $F \bar D$ is equal to the sum of degrees of all nodes, so $F = (n - 1)/(\bar D - 1)$.
Therefore, the space complexity is $2b(n - 1)/(\bar D - 1)$. % = 2b(n-1)/(bU - 1)$.
In order to compute an upper bound on the space complexity for a \bslack\ of height $h$, we simply need a lower bound on $\bar D$.
%Therefore, $S(n) = 2b(n - 1)/(\bar D - 1)$, which is related to utilization by $S(n) = 2b(n-1)/(bU - 1)$.
Above, we saw that $\bar D > b-2$ for \bslack s of height at least three.
It follows that a \bslack\ with $n > b^3$ keys %(which must have height at least three)
has space complexity at most $2b(n-1)/(b-3) < 2n \frac{b}{b-3}$.
\textbf{[[[Be VERY careful with the following... I think it's right, though.]]]}
A tighter upper bound is $2n \cdot b^{-1} \big( \frac{b\cdot d(h-1)-b+2}{b\cdot d(h-2)-b+3}-1 \big)$.

\textbf{[[[fix this]]]}
The full version of the paper describes pathological families of B-trees, Overflow trees and H-trees, and compares the space complexity of example trees in these families with the worst-case upper bound on the space complexity of a \bslack.
By studying these families, we obtain lower bounds on the space complexity of these trees that are above the upper bound for \bslack s.

We also study the number of rebalancing steps necessary to maintain balance in a \rbslack.
Consider a \rbslack\ obtained by starting from a \bslack\ containing $n$ keys and performing a sequence of $i$ insertions and $d$ deletions.
We prove that such a \rbslack\ will be transformed back into a \bslack\ after at most $2i(2 + \lfloor \log_{\lfloor\frac{b}{2}\rfloor} (n+i)/2 \rfloor) + d/(b-1)$ rebalancing steps, irrespective of which rebalancing steps are performed, and in which order.
Hence, insertions perform amortized $O(\log(n+i))$ rebalancing steps and deletions perform an amortized constant number of rebalancing steps.















%\subsection{Analysis of \bslack s} \label{sec-appendix-analysis}
%
%We analyze properties of \bslack s and \maxslack s with maximum degree $b$.
%A $(b,k)$-\maxslack\ is an \maxslack\ in which the root has degree $k$ and each node has maximum degree $b$.

\subsection{Analysis of \maxslack s} \label{sec-maxslack}

%We study properties of \bslack s and \maxslack s with maximum degree $b$.
For our analysis, it is helpful to generalize the definition of $b$-\maxslack s to the following.
A $(b,k)$-\maxslack\ is the same as $b$-\maxslack, except that the root has degree $k$, instead of degree two. % in which the root has degree $k$ and each node has maximum degree $b$.

%A tree in which the children of each internal node share exactly $b$ slack %(formally, for each internal node with children $v_1, v_2, ..., v_l$, $deg(v_1)+deg(v_2)+...+deg(v_l) = lb-b$) 
%is called a \textit{\maxslack}.
%A \maxslack\ with a root of degree $k \ge 2$ is called a \textit{$(b,k)$-\maxslack}.
%In this section, we prove several results about $(b,k)$-\maxslack s.
%In particular, we compute the total degree of nodes at each depth, and the average degree of nodes in a $(b,k)$-\maxslack\ of height $h$.
%As we will see, $(b,2)$-\maxslack s are very important for our analysis, because they represent the worst case for \bslack s in several respects.
%In Section~\ref{sec-maxslack-to-bslack}, we prove that a $(b,2)$-\maxslack\ has the greatest height of any \bslack\ containing the same number of keys, and the smallest average degree of nodes of any \bslack\ with the same height.

%We now prove several results about \maxslack s.
We now %Our first task is to 
compute the total degree of nodes at each depth in a $(b,k)$-\maxslack.
As we will see, for each $k$, the total degree of nodes at a given depth $\delta$ is the same in every $(b,k)$-\maxslack\ of height at least $\delta$.
%Recall that the degree of a leaf is the number of keys in the leaf.
%So, the following lemma also computes the number of keys in the leaves of a $(b,k)$-\maxslack.

\begin{lem} \label{lem-N}
%The number of pointers or keys at depth $\delta$ in a $(b,k)$-\maxslack\ is:
The total degree of nodes at depth $\delta$ in a $(b,k)$-\maxslack\ of height $h$ is:
 \begin{displaymath}
   d(\delta, k) = \left\{
     \begin{array}{ll}
       k & \mbox{if } \delta = 0 \\
       kb-b & \mbox{if } \delta = 1 \\
       b(d(\delta-1, k) - d(\delta-2, k))& \mbox{if } 1 < \delta \le h
     \end{array}
   \right.
  \end{displaymath}
\end{lem}
\begin{proof}
In the following, we use $c(u)$ to denote the set of children of node $u$.
Let %$k \ge 2$, and 
$T$ be a $(b,k)$-\maxslack.
The proof is by induction on $\delta$.
The base cases $\delta = 0$ and $\delta = 1$ are immediate from the definition of a $(b,k)$-\maxslack.
Consider $\delta > 1$.
Let $T_\delta$ be the set of nodes at depth $\delta$ in $T$.
Then, %$$|T_{\delta+1}| = 
$$d(\delta,k) = \sum_{v \in T_{\delta}} deg(v) = \sum_{u \in T_{\delta-1}} \sum_{v \in c(u)} deg(v).$$
Since $T$ is an \maxslack, $$\sum_{v \in c(u)} deg(v) = deg(u)b-b = b(deg(u)-1), \ \mbox{so}$$ $$d(\delta, k) = \sum_{u \in T_{\delta-1}} b(deg(u)-1) = b(d(\delta-1,k) - |T_{\delta-1}|) = b(d(\delta-1,k) - d(\delta-2,k)).$$
%Since the number of nodes at depth $\delta-1$ is equal to the total degree of nodes at depth $\delta-1$, we have $d(\delta,k) = b(d(\delta-1,k)-d(\delta-2,k)).$
\qed
\end{proof}

Since $d(\delta, k)$ is a linear homogeneous recurrence relation with constant coefficients, we use the technique described in Section~2.1.1(a) of \cite{greene1982mathematics} to obtain the following closed form solution.

\begin{lem} \label{lem-N-closed-form}
$d(\delta, k) = 2^{-\delta} (k_1 (b+\sqrt{b^2-4b})^{\delta} + k_2(b-\sqrt{b^2-4b})^{\delta}),$ where $k_1 = \frac{bk-2b}{2\sqrt{b^2-4b}} + \frac{k}{2}$ and $k_2 = k - k_1$.
\end{lem}
%\begin{proof}
\details{
We obtain a closed form solution for the recurrence %of Lemma~\ref{lem-nodes-at-depth-recurrence} 
using a technique described in Section~2.1.1(a) of \cite{greene1982mathematics}.
A linear homogeneous recurrence relation with constant coefficients is an equation of the form $a_n = c_1 a_{n-1} + c_2 a_{n-2} + ... + c_d a_{n-d}$.
The coefficients $c_1, ..., c_d$ yield the characteristic polynomial $p(t) = t^d - c_1 t^{d-1} - c_2 t^{d-2} - ... - c_d$.
If the roots $r_1, ..., r_d$ of $p(t)$ are unique, then $a_n = k_1 r_1^n + k_2 r_2^n + ... + k_d r_d^n$, where the coefficients $k_1, ..., k_d$ are chosen to satisfy the base cases for the recurrence.

Observe that $d(\delta) = b(d(\delta-1) - d(\delta-2))$ can be rewritten as $a_n = b a_{n-1} + (-b) a_{n-2}$, which yields the characteristic polynomial $p(t) = t^2 - bt + b$.
The quadratic equation yields roots $\frac{b \pm \sqrt{b^2 - 4b}}{2}$, which are unique for $b > 4$.
Thus, we have $a_n = k_1 \big(\frac{b + \sqrt{b^2 - 4b}}{2}\big)^n + k_2 \big(\frac{b - \sqrt{b^2 - 4b}}{2}\big)^n$.
Plugging in the base cases, we have $a_0 = k = k_1 + k_2$ and $a_1 = kb-b = k_1 \frac{b + \sqrt{b^2 - 4b}}{2} + k_2 \frac{b - \sqrt{b^2 - 4b}}{2}$.
The first equation yields $k_2 = k - k_1$.
After some basic algebra, %the second yields
$k_1 = \frac{kb - 2b}{2\sqrt{b^2-4b}} + \frac{k}{2}$.
%Clearly, $k_1 = k_2 = 1$ is a solution to both of these equations.
%\qed
}
%\end{proof}

\begin{cor} \label{cor-N-closed-form-two-maxslack}
$d(\delta, 2) = 2^{-\delta} ((b+\sqrt{b^2-4b})^{\delta} + (b-\sqrt{b^2-4b})^{\delta})$.
\end{cor}
%\begin{proof}
\details{
When $k=2$, $k_1 = \frac{bk-2b}{2\sqrt{b^2-4b}} + \frac{k}{2} = 1$ and $k_2 = k - k_1 = 1$.
}
%\qed
%\end{proof}

Since $b+\sqrt{b^2-4b}$ asymptotically approaches $2b$ as $b$ increases, and $b-\sqrt{b^2-4b}$ approaches zero, $d(\delta, 2)$ approximately grows like $b^{\delta}$ for large $b$.
%
%THE FOLLOWING IS WRONG. THIS NEEDS TO BE COMPUTED USING Dbar, NOT d!
%Simple algebra establishes the following bounds on $d(\delta, 2)$.
%\begin{cor} \label{cor-N-bounds}
%For $h \ge 3$, $\big(\frac{b}{2}\big)^h < (b-1.4)^h < (b-\frac{\gamma}{2})^h \le d(\delta, 2).$
%\end{cor}
Simple algebra establishes the following bounds on $d(\delta, 2)$.
\begin{cor} \label{cor-N-bounds}
For $h \ge 3$, $\big(\frac{b}{2}\big)^h < d(h, 2) \le b^h.$
\end{cor}

For the following lemma, we
%We
used symbolic mathematics software to obtain the partial derivatives of $d(\delta, k)$ with respect to $\delta$ and $k$, %.
%By proving that these derivatives are positive, we established the following lemmas.
and prove that they are positive.

\begin{lem} \label{lem-N-increasing-with-delta}
$d(\delta, k)$ is an increasing function of $\delta$ and $k$.
\end{lem}

%\details{
%\begin{lem} \label{lem-N-increasing-with-delta}
%$d(\delta, k)$ is an increasing function of $\delta$.
%\end{lem}
%%\begin{proof}
%We prove this claim by demonstrating that the partial derivative of $\bar D(\delta,k)$ with respect to $\delta$ is positive.
%This derivative (and several others that we will compute) would be difficult to obtain by hand, so we used symbolic mathematics software.
%The result was a function that we simplified to 
%$$\frac{\partial}{\partial\delta} d(\delta, k) = 2^{-\delta} \Big(k_1 \alpha^{\delta} \log_e \frac{\alpha}{2} + k_2 \gamma^{\delta} \log_e \frac{\gamma}{2} \Big),$$
%where $k_1$ and $k_2$ are defined as in Lemma~\ref{lem-N-closed-form}, $\alpha = b + \sqrt{b^2 - 4b}$, and $\gamma = b - \sqrt{b^2 - 4b}$.
%The result follows from a few facts, namely, $k_1 > 0$, $k_1 \ge k_2$ and $2 \le \gamma < \alpha$.
%These facts imply $k_1 \alpha^{\delta} > k_2 \gamma^{\delta}$ and $\log_e \frac{\alpha}{2} > \log_e \frac{\gamma}{2} \ge 0$, which proves the claim.
%%
%%We prove $d(\delta+1, k) > \frac{b}{b-1} d(\delta, k)$ for all $k \ge 2$ and $\delta \ge 0$ by induction on $\delta$.
%%Since $b \ge 5$, $kb-b \ge 4k > \frac{5}{4} k \ge \frac{b}{b-1} k$, so the claim holds for $\delta = 0$.
%%Suppose the claim holds for $\delta \ge 0$.
%%Then, $d(\delta+2, k) = b(d(\delta+1, k) - d(\delta, k)) > b(\frac{b}{b-1} d(\delta, k) - d(\delta, k)) = \frac{b}{b-1} d(\delta, k)$.
%%\trevor{There is a problem with this proof. I am only showing that the function increases every two steps of $\delta$...}
%%\qed
%%\end{proof}
%
%\begin{lem} \label{lem-N-increasing-with-k}
%$d(\delta, k)$ is an increasing function of $k$.
%\end{lem}
%%\begin{proof}
%We prove this claim by demonstrating $\frac{\partial}{\partial k} d(\delta, k) > 0$.
%Using our mathematics software, we obtained
%$$\frac{\partial}{\partial k} d(\delta, k) = \frac{\alpha^{\delta+1} - \gamma^{\delta+1}}{2^{\delta+1} \sqrt{b^2-4b}},$$
%where $\alpha = b + \sqrt{b^2 - 4b}$, and $\gamma = b - \sqrt{b^2 - 4b}$.
%Since $\alpha > \gamma$, $\frac{\partial}{\partial k} d(\delta, k) > 0$.
%%\qed
%%\end{proof}
%}

%The following observation is immediate from P\ref{prop-bslack-slack}.
%
%\begin{obs}
%Let $v$ be an internal node of degree $d$ in a \bslack.
%Since $b > 4$, it is possible to distribute the pointers or keys in $v$'s children such that each child has at least two pointers or keys.
%\end{obs}

\begin{lem} \label{lem}
The total degree of nodes in every $(b,k)$-\maxslack\ of height $h$ is
\begin{displaymath}
   D(h,k) = \left\{
     \begin{array}{ll}
       k & : h = 0 \\
       k + b(d(h-1,k)-1) & : h > 0
     \end{array}
   \right.
  \end{displaymath}
Moreover, $D(h, k)$ is increasing in $h$ and $k$.
\end{lem}
\begin{proof}
By Lemma~\ref{lem-N}, $D(h,k) = \sum_{\delta=0}^h d(\delta,k) = k + (kb-b) + \sum_{\delta=2}^h b(d(\delta-1,k)-d(\delta-2,k))$.
This telescoping sum reduces to $D(h,k) = k + (kb-b) + b(d(h-1,k)-d(0,k)) = k + b(d(h-1,k)-1)$.
Lemma~\ref{lem-N-increasing-with-delta} %and Lemma~\ref{lem-N-increasing-with-k}
implies that $D(h, k)$ is increasing in $h$ and $k$.
%The result follows from basic algebra. %Basic algebra yields $D(h,k) = b(d(h-1,k)-1)+3$.
\qed
\end{proof}

We now consider the average degree of nodes at each depth in a $(b,2)$-\maxslack.
In any $(b,2)$-\maxslack, the two children of the root must share exactly $2b-b = b$ pointers or keys.
Let us build intuition with an example.
Consider a $(b,2)$-\maxslack\ in which the children of the root evenly share $b$ pointers or keys.
The grandchildren of the root must share a total of exactly $((b/2)b-b) + ((b/2)b-b) = b^2-2b$ pointers or keys.
Thus, the average degree of nodes at depth zero is two, at depth one is $b/2$, and at depth two is $b-2$.
We prove that every $(b,2)$-\maxslack\ $T$ of height $h$ has the smallest average node degree of any $(b,k)$-\maxslack\ of height $h$.
We first derive expressions for the average degree of nodes in an \maxslack, and the average degree at each depth.

Since the total degree of nodes at depth $\delta$ is $d(\delta,k)$, and the total number of nodes at depth $\delta$ is $d(\delta-1,k)$, we obtain the following.

\begin{lem} \label{lem-d}
The average degree of nodes at depth $\delta$ in any $(b,k)$-\maxslack\ of height $h$ is:
\begin{displaymath}
   \bar d(\delta,k) = \left\{
     \begin{array}{ll}
       k & : \delta = 0 \\
       \frac{d(\delta,k)}{d(\delta-1,k)}& : 0 < \delta \le h
     \end{array}
   \right.
  \end{displaymath}
\end{lem}

We used our mathematics software to obtain the partial derivatives of $\bar d(\delta, k)$ with respect to $\delta$ and $k$.
We proved the following two lemmas by showing that $\frac{\partial}{\partial \delta} \bar d(\delta,k) > 0$ for $2 \le k \le b-2$, $\frac{\partial}{\partial \delta} \bar d(\delta,k) < 0$ for $k > b-2$, and $\frac{\partial}{\partial k} \bar d(\delta,k) > 0$.

\begin{lem} \label{lem-d-change-with-delta}
$\bar d(\delta,k)$ is an increasing function of $\delta$ for $2 \le k \le b-2$, and is a decreasing function of $\delta$ for $k \ge b-1$.
\end{lem}
\details%
{
\begin{proof}
We prove this lemma by demonstrating that the partial derivative of $\bar d(\delta,k)$ with respect to $\delta$ is positive for $2 \le k \le b-2$, and negative for $k > b-2$.
%This derivative would be extremely difficult to compute by hand, so we used a symbolic mathematics package.
%The result was a very complicated rational function that can be simplified to 
Using our mathematics software, we obtained a very complicated rational function that we simplified to 
$$\frac{\partial}{\partial \delta} \bar d(\delta,k) = \frac{-(k^2-bk+b)(4b)^{\delta} \sqrt{b^2-4b}\big(\alpha \gamma \log_e \frac{\alpha}{\gamma}\big)}{((2k-\gamma)(\alpha^{\delta}+\gamma^{\delta}))^2},$$
where $\alpha = b + \sqrt{b^2-4b}$ and $\gamma = b - \sqrt{b^2-4b}$.
Observe that $1 < \gamma < b < \alpha < 2b$.
Thus, the denominator is positive except when $2k - \gamma = 0$.
\trevor{Proving $2k-\gamma > 0$ is MUCH easier than this... Just use $\gamma < 2$.}
This is the case precisely when $k^2 - kb + b = 0$, which occurs when $k = \frac{\gamma}{2}$ or $k = \frac{\alpha}{2}$.
Since $b > 4$, $\frac{\gamma}{2} < 2$ and $b-2 < \frac{\alpha}{2} < b-1$.
\trevor{Where the hell did I get $b-2$ and $b-1$ from? Something seems wrong.}
Therefore, the denominator is always positive when $k \ge 2$. % is an integer.
Since $b \ge 5$, $4b > 0$ and $\sqrt{b^2-4b} > 0.$
Since $1 < \gamma < \alpha$, $\alpha\gamma\log_e \frac{\alpha}{\gamma} > 0$.
Therefore, $\frac{\partial}{\partial \delta} \bar d(\delta,k) > 0$ is equivalent to $k^2-bk+b < 0$.
As above, $k^2-bk+b = 0$ when $k=\frac{\gamma}{2}$ or $k=\frac{\alpha}{2}$.
For all $k \in (\frac{\gamma}{2}, \frac{\alpha}{2})$, $k^2-bk+b < 0$, so $\frac{\partial}{\partial \delta} \bar d(\delta,k) > 0$ for $2 \le k \le b-2$.
\trevor{Look at ``demonstrating that depthwise average degree is increasing with depth.nb'' to fix this proof.}
\qed
\end{proof}
}

\begin{lem} \label{lem-d-increasing-with-k}
$\bar d(\delta,k)$ is an increasing function of $k$.
\end{lem}
%%\begin{proof}
%\details{
%Using our symbolic mathematics package, we obtained %a rational function that simplified to
%$$\frac{\partial}{\partial k} \bar d(\delta,k) = \frac{4^{\delta+1}b^\delta (b-4)}{((2k-\gamma)(\alpha^{\delta}+\gamma^{\delta}))^2},$$
%where $\alpha = b + \sqrt{b^2-4b}$ and $\gamma = b - \sqrt{b^2-4b}$.
%As we argued above, the denominator is always positive when $k \ge 2$ is an integer.
%Thus, we need only show $4^{\delta+1}b^\delta (b-4) > 0$, which is true because $b \ge 5$.
%}
%%\qed
%%\end{proof}
%
%\begin{lem} \label{lem-d-lower-bound}
%$\bar d(\delta,k) \ge b-2$ for $2 \le \delta \le h$.
%\end{lem}
%\begin{proof}
%$\bar d(2,2) = \frac{d(2,2)}{d(1,2)} = \frac{b(2b-b - 2)}{2b-b} = b-2$.
%%$\bar d(2,k) = \frac{d(2,k)}{d(1,k)} = \frac{b(kb-b - b)}{kb-b} = \frac{b(k-1)-k}{k-1} = \frac{b(k-1)-(k-1)-1}{k-1} = \frac{(k-1)(b-1)}{k-1} = b-1-\frac{1}{k-1} \ge b-2$.
%By Lemma~\ref{lem-d-change-with-delta}, $\bar d(\delta,2) \ge b-2$ for $\delta \ge 2$.
%Finally, Lemma~\ref{lem-d-increasing-with-k} implies that $\bar d(\delta,k) \ge b-2$ for all $\delta,k \ge 2$.
%\qed
%\end{proof}

Let $T$ be a \bslack\ of height $h$.
Since every node in $T$ except for the root is pointed to by exactly one child pointer, the number of nodes in $T$ is the total degree of all nodes at depths zero through $h-1$, plus one for the root, which is exactly $D(h-1,k)+1$.
Thus, we obtain the following.

\begin{lem} \label{lem-D-closed-form}
The average degree of nodes in any $(b,k)$-\maxslack\ of height $h$ is:
 \begin{displaymath}
   \bar D(h,k) = \left\{
     \begin{array}{ll}
       k & : h = 0 \\
       \frac{D(h,k)}{D(h-1,k)+1}& : h > 0
     \end{array}
   \right.
  \end{displaymath}
\end{lem}
%\begin{proof}
%By definition, the average degree of nodes in $T$ is the total degree of nodes in $T$ divided by the number of nodes. %total space reserved for pointers in internal nodes and keys in leaves.
%The total degree of nodes in $T$ is exactly $D(h,k)$.
%Since every node except for the root is pointed to by exactly one child pointer, the number of nodes in $T$ is the total degree of all nodes at depths zero through $h-1$, plus one for the root.
%This is exactly $D(h-1,k)+1$.
%\qed
%\end{proof}

\begin{lem} \label{lem-D-change-with-h}
$\bar D(h,k)$ is an increasing function of $h$ for $2 \le k \le b-2$, and is a decreasing function of $h$ for $k \ge b-1$.
\end{lem}
\begin{proof}
%Fix $k$.
%Without loss of generality, suppose $k \le b-2$.
%(The argument is symmetric for $k > b-2$; simply negate every inequality and swap max and min.)
%The average degree of the nodes at depths zero through $h$ is the same in every $(b,k)$-\maxslack\ of height at least $h$.
%By definition, $\bar D(h,k)$ must be a weighted average of the terms $\bar d(0,k), \bar d(1,k), ..., \bar d(h,k)$.
%Thus, $\bar D(h+1,k)$ is a weighted average of $\bar D(h,k)$ and $\bar d(h+1,k)$
%By Lemma~\ref{lem-d-change-with-delta}, $\bar d(h+1,k) > \max_{i = 0...h} \bar d(i,k)$.
%Therefore, $\bar d(h+1,k) > \bar D(h,k)$, which implies that $\bar D(h+1,k) > \bar D(h,k)$.
%
The average node degree at depth $\delta \in \{0,1,...,h\}$ is the same in every $(b,k)$-\maxslack\ of height at least $h$.
By definition, $\bar D(h,k)$ must be a weighted average of the terms $\bar d(0,k), \bar d(1,k), ..., \bar d(h,k)$.
Thus, $\bar D(h+1,k)$ is a weighted average of $\bar D(h,k)$ and $\bar d(h+1,k)$
Suppose $k \le b-2$.
By Lemma~\ref{lem-d-change-with-delta}, $\bar d(h+1,k) > \max_{i \le h} \bar d(i,k)$.
Therefore, $\bar d(h+1,k) > \bar D(h,k)$, which implies that $\bar D(h+1,k) > \bar D(h,k)$.
Now, suppose $k \ge b-1$.
By Lemma~\ref{lem-d-change-with-delta}, $\bar d(h+1,k) < \min_{i \le h} \bar d(i,k)$.
Therefore, $\bar d(h+1,k) < \bar D(h,k)$, which implies that $\bar D(h+1,k) < \bar D(h,k)$.
\qed
\end{proof}

We used our mathematics software to obtain the partial derivative of $\bar D(h,k)$ with respect to $k$, and proved that it is positive, yielding the following result.

\begin{lem} \label{lem-D-increasing-with-k}
$\bar D(h,k)$ is an increasing function of $k$.
\end{lem}
%\begin{proof}
\details{
We prove $\frac{\partial}{\partial k} \bar D(h,k) > 0$.
As above, we used our mathematics software to compute the derivative, yielding a function that we simplified to
%This derivative would be extremely difficult to compute by hand, so we used a symbolic mathematics package.
%The result is a (very complicated) rational function.
$$\frac{\partial}{\partial k} \bar D(h, k) = \frac{2^h b(b-4)(2^{h+1} (1+b^{h+1}) - \alpha^{h+1} - \gamma^{h+1})}{((\gamma^h - \alpha^h)(\gamma(b+k) + 2b) + 2^{h+1}\sqrt{b^2-4b}(1+k-b))^2},$$
where $\alpha = b + \sqrt{b^2-4b}$ and $\gamma = b - \sqrt{b^2-4b}$.

We first prove that the numerator is positive.
Since $b > 4$, $2^h b(b-4) > 0$, so we need only prove %$2^{h+1}(1+b^{h+1}) > b \gamma^h - \gamma^h \sqrt{b^2-4b} + b \alpha^h + \alpha^h \sqrt{b^2-4b}$ or, equivalently, $2^{h+1}(1+b^{h+1}) > \gamma^h (b - \sqrt{b^2-4b}) + \alpha^h (b + \sqrt{b^2-4b})$.
%Substituting $\alpha$ and $\gamma$, we obtain
$2^{h+1}(1+b^{h+1}) > \alpha^{h+1} + \gamma^{h+1}$.
By the binomial theorem, $(\alpha + \gamma)^{h+1} = \sum_{k=0}^{h+1} \binom{h+1}{k} \alpha^{(h+1)-k} \gamma^k = \alpha^{h+1} + \gamma^{h+1} + \sum_{k=1}^h \binom{h}{k} \alpha^{h-k} \gamma^k$.
Since $\alpha + \gamma = 2b$, $(2b)^{h+1} = \alpha^{h+1} + \gamma^{h+1} + \sum_{k=1}^h \binom{h}{k} \alpha^{h-k} \gamma^k \ge \alpha^{h+1} + \gamma^{h+1}$.
Since $2^{h+1}(1+b^{h+1}) > (2b)^{h+1}$, we have established $2^{h+1}(1+b^{h+1}) > \alpha^{h+1} + \gamma^{h+1}$. %, which proves that $\frac{\partial}{\partial k} \bar D(h,k) > 0$.

We now prove that the denominator is positive.
Since the denominator is of the form $(f(k))^2$, it suffices to prove $f(k) = (\gamma^h - \alpha^h)(\gamma(b+k) + 2b) + 2^{h+1}\sqrt{b^2-4b}(1+k-b) \neq 0$.
We first try to show $f(k) < 0$.
Since $\gamma < \alpha$ and $\gamma, b, k > 0$, $(\gamma^h - \alpha^h)(\gamma(b+k) + 2b) < 0$.
The expression $2^{h+1}\sqrt{b^2-4b}$ is positive, so $f(k) < 0$ will be true if $k \le b-1$.
Suppose $k = b$.
Then, $f(k) = f(b) = \alpha^h - \gamma^h - 2^{h-1} \sqrt{1-4/b}$.
We prove $f(b) > 0$.
Since $b > 4$, $f(b) > \alpha^h - \gamma^h - 2^{h-1}$.
By the binomial theorem, $2^{h-1} + \gamma^h < 2^h + \gamma^h < (2+\gamma)^h$.
Observe that $\alpha > \gamma+2$.
Thus, $2^{h-1} + \gamma^h < (2+\gamma)^h < \alpha^h$, so $f(b) > 0$.
Therefore, in all cases, $f(k) \neq 0$.
}
%\qed
%\end{proof}

We proved a simple lower bound on $\bar D(h,k)$ using our mathematics software.

\begin{lem} \label{lem-D-lower-bound}
%$\bar D(h,k) \ge b-4$ for $h = 2$, and
$\bar D(h,k) > b-2$ for $h \ge 3$ (and $b \ge 5$).
\end{lem}
%\begin{proof}
%Simple algebra checked by our mathematics software.%a theorem prover.
%\qed
%\end{proof}

%%\begin{lem} \label{lem-d-increases-with-depth}
%%$\bar d(\delta,k)$ is an increasing function of $\delta$ for $2 \le k \le b-2$, and is a decreasing function of $\delta$ for $k > b-2$.
%%\end{lem}
%%\begin{proof}
%%We prove this lemma by demonstrating that the partial derivative of $\bar d(\delta,k)$ with respect to $\delta$ is positive for $2 \le k \le b-2$, and negative for $k > b-2$.
%%This derivative would be extremely difficult to compute by hand, so we used a symbolic mathematics package.
%%The result is a (very complicated) rational function.
%%Since we are only interested in showing $\frac{\partial}{\partial \delta} \bar d(\delta,k) > 0$, we need only consider the numerator, which is
%%$$-(k^2-bk+b)(4b)^{\delta} \sqrt{b^2-4b}\Big(\alpha \gamma \log_e \frac{\alpha}{\gamma}\Big),$$
%%where $\alpha = b + \sqrt{b^2-4b}$ and $\gamma = b - \sqrt{b^2-4b}$.
%%Observe that $1 < \gamma < b < \alpha < 2b$.
%%Thus, $\frac{\partial}{\partial \delta} \bar d(\delta,k) > 0$ is equivalent to $k^2-bk+b < 0$.
%%The roots of $k^2-bk+b$ are $\frac{\gamma}{2}$ and $\frac{\alpha}{2}$.
%%For all $k \in (\frac{\gamma}{2}, \frac{\alpha}{2})$, $k^2-bk+b < 0$ is satisfied.
%%The result follows from the fact that $\frac{\gamma}{2} < 2$ and $b-2 < \frac{\alpha}{2} < b-1$ when $b > 4$.
%%\qed
%%\end{proof}
%
%\begin{cor} \label{cor-D-increases-with-depth}
%$\bar D(h,k)$ is an increasing function of $h$ for $2 \le k \le b-2$, and is a decreasing function of $h$ for $k > b-2$.
%\end{cor}
%\begin{proof}
%Fix $k$.
%Without loss of generality, suppose $k \le b-2$.
%(The argument is symmetric for $k > b-2$; simply flip every inequality and swap max and min.)
%The average degree of the nodes at depths zero through $h$ is the same in every $(b,k)$-\maxslack.
%By definition, $\bar D(h,k)$ is a weighted average of the terms $\bar d(0,k), \bar d(1,k), ..., \bar d(h,k)$.
%Thus, $\bar D(h+1,k)$ is a weighted average of $\bar D(h,k)$ and $\bar d(h+1,k)$
%By Lemma~\ref{lem-d-increases-with-depth}, $\bar d(h+1,k) > max_{i \le h} \bar d(i,k)$.
%Therefore, $\bar d(h+1,k) > \bar D(h,k)$, which implies that $\bar D(h+1,k) > \bar D(h,k)$.
%%
%%Let $T$ be a $(b,k)$-\maxslack\ of height $h+1$.
%%Lemma~\ref{lem-d-increases-with-depth} implies that $\bar d(h+1,k) > max_{i \in \{0,1,...,h\}} \bar d(i,k)$.
%%The average degree of the nodes of $T$ at depths zero through $h$ is $\bar D(h,k)$.
%%By definition, $\bar D(h,k)$ is a weighted average of the average degrees of nodes at depths zero through $h$.
%%Therefore, $max_{i \in \{0,1,...,h\}} \bar d(i,k) \ge \bar D(h,k)$.
%%
%%Therefore, adding the final level of nodes to $T'$ 
%%%Immediate from Lemma~\ref{lem-d-increases-with-depth} and the fact that the first $h$ levels of a $(b,k)$-\maxslack\ of height $h+1$ form a $(b,k)$-\maxslack\ of height $h$.
%\qed
%\end{proof}
%
%$\bar D(h,k)$ does not, in fact, increase with $h$ for $k > b-2$.
%One can show that $\bar D(h,b-1) = b-1$, and $b-1 < \bar D(h+1,b) < \bar D(h,b)$.
%\trevor{I suppose this should be a lemma--maybe part of Corollary~\ref{cor-D-increases-with-depth}.  (Actually, this should probably be propagated back into Lemma~\ref{lem-d-increases-with-depth}.)}
%
%\begin{lem} \label{lem}
%%$\bar D(h,k) \ge b-1$ for $k > b-2$, and
%$\bar D(h,k) \ge b-4$ for $h \ge 2$, and $\bar D(h,k) \ge b-2$ for $h \ge 3$.
%\end{lem}
%\begin{proof}
%Simple algebra checked by our symbolic mathematics package.%a theorem prover.
%\qed
%\end{proof}
%
%\begin{lem} \label{lem}
%$\bar D(h,k)$ is an increasing function of $k$.
%\end{lem}
%\begin{proof}
%We prove $\frac{\partial}{\partial k} \bar D(h,k) > 0$.
%As above, we used our symbolic mathematics package to compute the derivative, yielding the numerator: \trevor{WARNING: THE DENOMINATOR NEEDS TO BE POSITIVE!!!!!!!!!!!!!!!}
%%This derivative would be extremely difficult to compute by hand, so we used a symbolic mathematics package.
%%The result is a (very complicated) rational function.
%$$2b(b-4)(2^{h+1}(1+b^{h+1}) + \gamma^h \sqrt{b^2-4b} - \alpha^h \sqrt{b^2-4b} - b \gamma^h - b \alpha^h),$$
%where $\alpha = b + \sqrt{b^2-4b}$ and $\gamma = b - \sqrt{b^2-4b}$.
%Since $b > 4$, $2b(b-4) > 0$.
%We thus prove $2^{h+1}(1+b^{h+1}) > b \gamma^h - \gamma^h \sqrt{b^2-4b} + b \alpha^h + \alpha^h \sqrt{b^2-4b}$ or, equivalently, $2^{h+1}(1+b^{h+1}) > \gamma^h (b - \sqrt{b^2-4b}) + \alpha^h (b + \sqrt{b^2-4b})$.
%Substituting $\alpha$ and $\gamma$, we obtain $2^{h+1}(1+b^{h+1}) > \alpha^{h+1} + \gamma^{h+1}$.
%By the binomial theorem, $(\alpha + \gamma)^{h+1} = \sum_{k=0}^{h+1} \binom{h+1}{k} \alpha^{(h+1)-k} \gamma^k = \alpha^{h+1} + \gamma^{h+1} + \sum_{k=1}^h \binom{h}{k} \alpha^{h-k} \gamma^k$.
%Since $\alpha + \gamma = 2b$, $(2b)^{h+1} = \alpha^{h+1} + \gamma^{h+1} + \sum_{k=1}^h \binom{h}{k} \alpha^{h-k} \gamma^k \ge \alpha^{h+1} + \gamma^{h+1}$.
%Since $2^{h+1}(1+b^{h+1}) > (2b)^{h+1}$, we have established $2^{h+1}(1+b^{h+1}) > \alpha^{h+1} + \gamma^{h+1}$, which proves that $\frac{\partial}{\partial k} \bar D(h,k) > 0$.
%\qed
%\end{proof}


































\subsection{Relating \bslack s to \maxslack s} \label{sec-maxslack-to-bslack}

In this section, we first prove that a $(b,2)$-\maxslack\ has the greatest height of any \bslack\ containing the same number of keys, and a smaller average degree of nodes than any \bslack\ with the same height.
Then, we compute upper and lower bounds on the space used to store a \bslack\ with $n$ keys.

%%In the following, we use $d(\delta)$ as shorthand for $d(\delta, 2)$.
%We now prove that any $(b,2)$-\maxslack s has the minimum total degree, at each depth, of any \bslack\ of the same height.
%Since the degree at the lowest depth of the tree is simply the number of keys in the tree, this yields an immediate height bound for \bslack s.

\begin{prop} \label{lem-internal-with-slack-has-degree-three-child}
Let $u$ be an internal node in a \bslack. %\ with children $v_1, v_2, ..., v_l$.
If the total slack contained in the children of $u$ is less than $b$, then some child of $u$ has degree at least three.
%If $deg(v_1)+deg(v_2)+...+deg(v_l) > lb-b$, then some $v_i$ has degree at least three.
\end{prop}
\begin{proof}
Suppose the total slack contained in the children $v_1, v_2, ..., v_l$ of $u$ is less than $b$.
Then, $deg(v_1)+deg(v_2)+...+deg(v_l) > lb-b$.
By P\ref{prop-bslack-internal}, $l \ge 2$.
Since $b > 4$, it follows that $lb-b = b(l-1) > 4(l-1) \ge 2l$.
Therefore, the average degree of the children of $u$ is $(deg(v_1)+deg(v_2)+...+deg(v_l))/l > \frac{lb-b}{l} > 2$.
\qed
\end{proof}

\begin{lem} \label{lem-N-worst-in-two-maxslack}
Every $(b,2)$-\maxslack\ of height $h$ has a smaller total degree of nodes, at each depth, than any \bslack\ of height $h$.
%Every $(b,2)$-\maxslack\ of height $h$ contains the minimum number of keys of any \bslack\ of height $h$. % Every \bslack\ $T$ of height $h$ that contains the minimum number of keys of any tree of height $h$ is a $(b,2)$-\maxslack.
\end{lem}
\begin{proof}
Let $T$ be a \bslack\ of height $h$. % that is not a $(b,2)$-\maxslack.
We can transform $T$ into a $(b,2)$-\maxslack\ by removing keys and pointers.
Removing a key, or a pointer from a node that has at least three pointers, does not affect P\ref{prop-bslack-depth}, P\ref{prop-bslack-internal} or P\ref{prop-bslack-leaf}.
%Since $T$ is not a $(b,2)$-\maxslack, for some internal node $u$, the total slack contained in the children of $u$ is less than $b$.
Let $u$ be any internal node whose children share a total of less than $b$ slack.
We arbitrarily remove a key or pointer from the child, $v$, of $u$ with the largest degree.
By Proposition~\ref{lem-internal-with-slack-has-degree-three-child}, $v$ must have degree at least three.
%Removing a key or pointer from $v$ increases the total slack contained in the children of $u$ by one, so it does not violate P\ref{prop-bslack-slack}.
%Therefore, $T$ is still a \bslack.
We can repeat this process until $T$ is a $(b,2)$-\maxslack.
\qed
\end{proof}

\begin{cor} \label{cor-2maxslack-worst-case-height}
Every $(b,2)$-\maxslack\ with $n$ keys has a larger height than any \bslack\ with $n$ keys.
\end{cor}

\begin{cor} \label{cor-2maxslack-fewest-keys}
Any \bslack\ of height $h$ contains more keys than every $(b,2)$-\maxslack\ of height $h$, and, hence, more than $d(h,2)$ keys.
\end{cor}

\begin{lem} \label{lem-D-lower-bound-for-bslack}
Every $(b,2)$-\maxslack\ of height $h$ has a smaller average node degree than any \bslack\ of height $h$.
\end{lem}
\begin{proof}
We first describe how to transform a \bslack\ into an \maxslack\ of the same height while decreasing the average node degree.
Observe that, since an \maxslack\ satisfies P\ref{prop-bslack-depth}, P\ref{prop-bslack-internal} and P\ref{prop-bslack-leaf}, any \bslack\ will become an \maxslack\ if pointers and keys are removed until, for each internal node $u$, the children of $u$ share a total of $b$ slack.
%The high-level idea 
%%of the transformation 
%is to start at the parents of leaves, and work up towards the root, level by level.
%At each step, we remove some keys or pointers to transform an internal node of degree $k$ whose children are either leaves, or the roots of \maxslack s, into the root of a $k$-maxslack tree.
%Every time we remove a pointer, we must ensure that we do not increase the average node degree.
%
The proof is by induction on the height of the tree.
Let $u$ be the root of a \bslack\ $T$. % and $v_1, v_2, ..., v_l$ be its children.

In the base case, the children of $u$ are leaves.
Arbitrarily removing keys from the children of $u$ until the children contain a total of exactly $b$ slack will transform $T$ into an \maxslack\ while decreasing the average degree of nodes.

Now, suppose the children of $u$ are internal.
By the inductive hypothesis, we can transform each subtree rooted at a child of $u$ into an \maxslack.
After these transformations, for every internal node in every subtree rooted at a child of $u$, the children of this internal node contain a total of $b$ slack.
If the children of $u$ contain a total of $b$ slack, then $T$ is an \maxslack.
Otherwise, we would like to remove some grandchild of $u$, to increase this slack.
%(If we increase this slack to $b$, then $T$ will be an \maxslack.)
As we argued in the proof of Lemma~\ref{lem-N-worst-in-two-maxslack}, removing a pointer from a node that has the largest degree amongst its siblings yields a \bslack. %does not affect P\ref{prop-bslack-depth}, P\ref{prop-bslack-internal}, P\ref{prop-bslack-leaf} or P\ref{prop-bslack-slack}.
However, we must carefully choose which grandchild to remove so that we decrease the average degree of nodes.
%
%More specifically, we removing the grandchild that is the root of the tree with the largest average node degree, we can avoid increasing the average node degree.
%To avoid increasing the average node degree, we must remove the grandchild that is the root of the tree with the largest average node degree.
%However, removing a node could increase the average degree of nodes, so we must carefully choose which grandchild to remove.
Let $v$ be the child of $u$ that is the root of the tree with the largest average degree.
By Lemma~\ref{lem-D-increasing-with-k}, $v$ has the largest degree amongst its siblings.
By Lemma~\ref{lem-internal-with-slack-has-degree-three-child}, $v$ must have at least three pointers, so removing one of its children does not violate P\ref{prop-bslack-internal}.
It is easy to verify that removing one of $v$'s children will not violate P\ref{prop-bslack-depth} or P\ref{prop-bslack-leaf}.
We remove the child of $v$ that is the root of the tree with the largest average degree.
Since this tree 
%the tree rooted at $w$ 
has the largest average degree of any tree rooted at a child of $v$, removing it decreases the average degree of $T$. %the tree rooted at $v$.
(This is because every other subtree rooted at a child of $v$ has the same or smaller average degree, and removing this child of $v$ decreases the degree of $v$.)
%Since the average degree of the tree rooted at $v$ does not increase, neither does the average degree of $T$.
%Each child of $r$ is still the root of an \maxslack, because removing a pointer does not decrease the slack of any node.
%
%It is easy to verify that each child of $r$ is still the root of an \maxslack.
We can repeatedly apply this transformation until the children of $u$ contain a total of $b$ slack, at which point $T$ is an \maxslack.

We now prove the main result.
Given a \bslack\ $T$, we first transform it into an \maxslack.
Then, if the root of $T$ has more than two children, we transform $T$ into a $(b,2)$-\maxslack\ by keeping the two children %of the root 
that are the roots of the trees with the largest average degrees, and throwing away the rest.
\qed
\end{proof}

%We now prove that every $(b,2)$-\maxslack\ of height $h$ has the minimum average node degree of any \bslack\ of height $h$.
%The proof of the following lemma describes how to transform a \bslack\ of a special form into an \maxslack\ of the same height without increasing the average degree of nodes.
%The subsequent corollary uses this lemma to transform any \bslack\ into a $(b,2)$-\maxslack\ of the same height without increasing the average degree of nodes.
%The high-level idea of the transformation is to start at the parents of leaves, and work up towards the root, level by level.
%At each step, it transforms an internal node of degree $k$ whose children are either leaves, or the roots of \maxslack s, into the root of a $k$-maxslack tree.
%Finally, if the root of the entire tree has more than two children, we carefully remove all but two to obtain a $(b,2)$-\maxslack.

%\begin{lem} \label{lem-average-degree-inductive-step}
%Let $T$ be any \bslack\ that is not an \maxslack, and such that the children of the root are either leaves or the roots of \maxslack s.
%Then, $T$ can be transformed into an \maxslack\ of the same height without increasing the average degree of nodes.
%\end{lem}
%\begin{proof}
%Let $r$ be the root of $T$ and $v_1, v_2, ..., v_l$ be its children.
%
%Suppose the children of $r$ are leaves.
%Arbitrarily removing keys from the children of $r$ until $lb-b$ remain will transform $T$ into an \maxslack\ without increasing the average degree of nodes.
%
%Now, suppose the children of $r$ are internal.
%Since $T$ is not an \maxslack, there is some internal node with less than $b$ slack shared amongst its children.
%Since each child of $r$ is the root of an \maxslack, for every internal node that is not the root, exactly $b$ slack is shared amongst its children. %the root is the only such internal node whose children share less than $b$ slack. %for each internal node that is not the root, exactly $b$ slack is shared amongst its children.
%%$T$ the only thing that prevents $T$ from being an \maxslack\ is the fact that $v_1, v_2, ..., v_{|c(r)|} > |c(r)|b-b$.
%Therefore, the root is the only node with less than $b$ slack shared amongst its children.
%%$v_1 + v_2 + ... + v_{|c(r)|} > |c(r)|b-b$.
%%
%%Since $T$ is not a maxslack tree, there is some internal node $u$ with children $v_1, v_2, ..., v_{|c(u)|}$ such that $deg(v_1)+...+deg(v_{|c(u)|}) > |c(u)|b-b$.
%%Formally, $deg(v_1) + deg(v_2) + ... + deg(v_l) > lb-b$.
%We would like to remove some grandchild of $r$, to increase this slack. %reduce the left side of this inequality.
%However, removing a node could violate P\ref{prop-bslack-internal} or increase the average degree of nodes, so we must carefully choose which node to remove.
%Let $v_i$ be the child of $r$ that is the root of the tree with the largest average degree.
%By Lemma~\ref{lem-D-increasing-with-k}, $v_i$ must have the largest degree of any child of $r$.
%%
%By Lemma~\ref{lem-internal-with-slack-has-degree-three-child}, $v_i$ must have at least three pointers.
%%As we proved above, since $b > 4$ and $|c(r)| \ge 2$, for every internal node $u$, $deg(v_1)+...+deg(v_{|c(u)|}) > |c(u)|b-b \ge 2|c(u)|$, so some child of $r$ must have at least three pointers.
%%Since $d_1+…+d_d > db-b$, Observation~\ref{missing-obs} implies that some child of v has at least three pointers.
%%Therefore, $v_i$ must have at least three pointers.
%Let $w$ be the child of $v_i$ that is the root of the tree with the largest average degree.
%Since the tree rooted at $w$ has the largest average degree of any tree rooted at a child of $v_i$, removing it will not increase the average degree of the tree rooted at $v_i$.
%Since the average degree of the tree rooted at $v_i$ will not increase, neither will the average degree of $T$.
%Thus, we can safely remove $w$ from the tree.
%It is easy to verify that each child of $r$ is still the root of an \maxslack.
%Clearly, we can repeatedly apply this transformation until $deg(v_1)+...+deg(v_l) = lb-b$, at which point $r$ will be the root of an \maxslack.
%\qed
%\end{proof}
%
%\begin{cor}
%Every \bslack\ of height $h$ can be transformed into a $(b,2)$-\maxslack\ of the same height without increasing the average degree of nodes.
%%Every $(b,2)$-\maxslack\ of height $h$ has the minimum average node degree of any \bslack\ of height $h$.
%\end{cor}
%\begin{proof}
%Let $T$ be any \bslack, and $k$ be the degree of the root.
%Using Lemma~\ref{lem-average-degree-inductive-step}, we can transform $T$ $(b,k)$-\maxslack\ by starting at the parents of leaves, and working our way up the tree, level by level.
%Finally, we can transform the $(b,k)$-\maxslack\ into a $(b,2)$-\maxslack\ by keeping the two children of the root that are the roots of the trees with the largest average degree, and throwing away the rest.
%Note that this transformation does not increase the average degree of nodes.
%\qed
%\end{proof}

Since the average degree of nodes represents the fraction of space that is utilized, this %result also 
implies that every $(b,2)$-\maxslack\ of height $h$ wastes a larger proportion of space than any \bslack\ of the same height.
We can also obtain a lower bound on the average degree (and, hence, the fraction of space that is utilized) for any \bslack\ containing $n$ keys.

\begin{lem} \label{lem-2maxslack-worst-case-Dbar}
A \bslack\ with $n \ge 2$ keys has average degree greater than $\bar D(\lceil \log_b n \rceil - 1, 2)$.
\end{lem}
\begin{proof}
Let $T$ be a \bslack\ of height $h$ containing $n$ keys.
By Lemma~\ref{lem-D-lower-bound-for-bslack}, $T$ has average degree greater than $\bar D(h,2)$.
Lemma~\ref{lem-D-change-with-h} implies that $\bar D(h,2)$ increases with $h$, so it suffices to find a lower bound on $h$.
Since $b$ is the maximum possible degree for any node in $T$, $h$ is at least $\lceil \log_b n \rceil - 1$.
%If every node in $T$ has the maximum possible degree, $b$, then $n = b^{h+1}$, so $h = \lceil \log_b n \rceil - 1$.
%It follows that the height of $T$ is at least $\lceil \log_b n \rceil - 1$.
\qed
\end{proof}

We can now compute bounds on $\func{S}(n)$, the space complexity of a \bslack\ containing $n$ keys.
%$\func{S}(n)$ is the total number of words of memory occupied by all nodes.
%To simplify this computation, we assume keys and pointers each occupy a single word in memory.
%The number of words occupied by a node is then $2b$.
%(Technically, internal nodes use up to $2b-1$ words, but we are assuming only one block size can be allocated.)
%%The number of words occupied by a node is then $2b-1$ for internal nodes %($b$ pointers and $b-1$ keys) 
%%and $2b$ for leaves. %($b$ pointers and $k$ keys).
%Therefore, $\func{S}(n) = 2bF$, where $F$ is the total number of nodes in the tree.
Recall from Section~\ref{sec-bslack} that $\func{S}(n) = 2b(n-1)/(\bar D - 1)$.
%We can obtain an upper bound on $F$ by using the lower bound on average degree that was derived above.
%By definition, the total degree of the tree is $F - 1 + n$, since each node has a pointer into it, except for the root, and the degree of a leaf is the number of keys it contains.
%Let $D^* \le b$ be the average degree of the tree.
%Then, $F D^*$ is equal to the total degree, $F - 1 + n$, so $F = \frac{n - 1}{D^* - 1}$.
%%Therefore, $F$ is maximized when average degree is minimized.
By Lemma~\ref{lem-2maxslack-worst-case-Dbar}, $D^* \ge \bar D(\lceil \log_b n \rceil - 1, 2)$.
Let $s = \bar D(\lceil \log_b n \rceil - 1, 2)$.
Then, $$\frac{n-1}{b-1} \le F \le \frac{n-1}{s - 1} \ \mbox{ and } \ \frac{2b(n-1)}{b-1} \le \func{S}(n) \le \frac{2b(n-1)}{s - 1}.$$
%We can also obtain an upper bound that is looser, but somewhat easier to understand.
%When $n > b^3$, $\lceil \log_b n \rceil - 1 \ge 3$, so Lemma~\ref{lem-D-lower-bound} implies $s > b-1.4$.
%Therefore, $\func{S}(n) < \frac{2b(n-1)}{b-2.4} < \frac{2b}{b-2.4}n$.
%
\\

%\trevor{Do a comparison of average degree and S for \bslack s and B-trees (and maybe others) for some concrete parameters such as $b=5, 16, 32$.}

%\trevor{Possibly show experimental results that hopefully indicate an amortized constant number of rebalancing steps. (Run the same workload for increasing tree sizes, and plot the number of rebalancing steps per update.)}

%\trevor{Full paper: compute space per key for differing key and pointer sizes.
%Also do this for a set ADT (so that each leaf contains at most $2b-1$ keys and no pointers)?}

%\trevor{Want: every $(b,2)$-\maxslack\ with $n$ keys wastes the largest proportion of space of any \bslack\ with $n$ keys... wait... this seems to be false... what can we say? algorithmically, users can look at a desired key count, take its logarithm base $b$, then find the smallest height the tree could be, and compute the average node degree for a $(b,2)$-\maxslack\ of that height. can i come up with something better than this?
%To formalize the algorithm, I think: a \bslack\ with $n \ge 2$ keys has average degree at least $\bar D(\lceil \log_b n \rceil-1,2)$. I would have liked average degree at least $\bar D(h,2)$. Unfortunately, $\lceil \log_b n \rceil - 1$ can be somewhat smaller than $h$.}

%\begin{cor}
%Every $(b,2)$-\maxslack\ of height $h$ wastes the largest proportion of space of any \bslack\ of height $h$.
%\end{cor}

%\begin{lem}
%Suppose $T$ is a $(b,k)$-\maxslack\ of height $h \ge 2$, where $k > 2$, and $T'$ is the tree obtained from $T$ by removing the $b$ grandchildren of the root with the largest degrees. %, where the children of the root have degrees $d_1, d_2, ..., d_k$, respectively.
%Then, $T'$ is a $(k-1)$-\maxslack\ of height $h$, and the average degree of nodes in $T'$ is the same as, or smaller than, the average degree of nodes in $T$.
%\trevor{This is still wrong.  We are not removing a child of the root, so $k$ is not decreasing...}
%\end{lem}
%\begin{proof}
%Let $d_1, d_2, ..., d_k$ be the degrees of the children of the root of $T$, and $v$ be the child with the largest degree, $d_i$.
%Clearly, removing $v$ does not affect P\ref{prop-bslack-depth} and P\ref{prop-bslack-leaf}.
%Since $k > 2$, P\ref{prop-bslack-internal} is still satisfied after $v$ is removed.
%It remains to show that P\ref{prop-bslack-slack} holds after $v$ is removed.
%Equivalently, we must show $d_1 + d_2 + ... + d_{i-1} + d_{i+1} + ... + d_k = (k-1)b - b$.
%
%it's not v we're removing... it's the grandchildren of the root...
%%This follows immediately from $d_i \le b$ and the fact that $d_1 + d_2 + ... + d_k = kb - b$ was satisfied before $v$ was removed.
%
%\end{proof}


























\subsection{Amortized logarithmic rebalancing} \label{sec-log-rebalancing}

%%
%%In practice, 
%In the worst-case, $Br(T,\delta) \le b-1$, since a tree $T$ in which every node has $b-1$ children is a \bslack.
%Beyond depth two, $Br(T,\delta)$ quickly closes the gap between $b-2$ and its worst-case upper bound of $b-1$.
%For instance, in a $16$-slack tree $T$, where $Br(T,\delta) \le 15$ in the worst-case, $Br(T,3) \approx 14.86$ and $Br(T,4) \approx 14.92$.
%Note that %Since the children of each internal node can share $b$ slack, 
%$Br(T, \delta) \le b-1$ in the worst-case, since the children of each internal node can share $b$ slack.
%Interestingly, the average node degree in every \bslack increases quite quickly with depth, exceeding $b-2$ at depth three.
% 
%that, as the depth of a node goes to $\infty$, the number of pointers or keys shared \textit{among its children} goes to $b^2-b$ (which implies that the average number of pointers or keys per node goes to $b-1$).


%We now prove that every \rbslack\ can be transformed into a \bslack\ by performing a finite number of rebalancing steps.  (We prove amortized logarithmic rebalancing in Section~\ref{sec-analysis}.)
%%, and that at most an amortized logarithmic number of rebalancing steps is needed to do this transformation.
%Note that any results proved for \rbslack s also hold for \bslack s.

In the following, we assume that the tree is initially a \bslack.
After a sequence of insertions and deletions, the tree is a \rbslack.
The goal of this section is to establish an upper bound on the number of rebalancing steps needed to transform this \rbslack\ back into a \bslack.

We assume that the updates shown in Figure~\ref{fig-updates} are performed sequentially.
In a concurrent setting, locks or non-blocking techniques such as \cite{paper2} can be used to ensure that updates appear to atomically operate on mutually exclusive sets of nodes (so that the effect will be the same as if the updates were performed sequentially in some order).

Our analysis follows the approach taken in \cite{LF95}, starting from any \bslack.
Initially, we associate every key in the tree with the leaf that contains it.
When a key is inserted into a leaf $u$, we associate the key with $u$.
After a key is deleted from $u$, the key is still associated with $u$.
If the node $u$ is deleted, then all keys associated with $u$ are instead associated with another node.
Two cases arise.
If $u$ is deleted by a Root-Replace, then all keys associated with $u$ are instead associated with the only child of $u$.
Otherwise, $u$ is deleted by Absorb or Compress, and all keys associated with $u$ are instead associated with the parent of $u$ before the Absorb or Compress.

Let $T$ be a \bslack, $\sigma$ be a sequence of updates to $T$, and $w$ be an internal node in the tree after the updates in $\sigma$ have been performed.
We define the \textit{\iset} of $w$ to be the multiset of all keys associated with nodes in the subtree rooted at $w$.
Therefore, the \iset\ of the root contains $n+i$ keys, where $i$ is the number of insertions that are performed on the initial \bslack\ and $n$ is the size of $T$.

We also define the \textit{relaxed height} of a node $u$ in a \rbslack.
Suppose we formed a new \rbslack\ $T$ by detaching the subtree rooted at $u$ from the \rbslack\ that contains it. %Consider the \rbslack\ $T$ that would be formed by detaching the subtree rooted $u$ from the \rbslack\ that contains it.
Then, the relaxed height of $u$, denoted $rh(u)$, is the relaxed depth of the leaves in $T$.

The following lemma relates the relaxed height of a node to the number of keys in its \iset.

\begin{lem}
Consider a \bslack\ $T$ containing at least two keys, and a sequence of updates to it.
Then, let $u$ be any node in the resulting tree.
If $u$ is the root, then its \iset\ contains at least $2 \big\lfloor \frac b 2 \big\rfloor^{rh(u)-weight(u)}$ keys.
Otherwise, its \iset\ contains at least $\big\lfloor \frac b 2 \big\rfloor^{rh(u)}$ keys.
\end{lem}
\begin{proof}
The proof is by induction on the sequence of updates performed on $T$.

\textbf{Base case.}
Let $u$ be any node in $T$, $T_u$ be the tree rooted at $u$, and $h_u$ be the height of $T_u$.
Any subtree of a \bslack\ is a \bslack, so $T_u$ is a \bslack.
By Corollary~\ref{cor-2maxslack-fewest-keys}, $T_u$ must contain at least $d(h_u,2)$ keys.
By Corollary~\ref{cor-N-bounds}, $d(h_u,2) > (\frac b 2)^{h_u}$.
Since $T_u$ is a \bslack, every node has \weight\ one, so the relaxed height of each node is equal to its height and $h_u = rh(u)$.
Therefore, $d(h_u,2) > (\frac b 2)^{rh(u)} \ge \lfloor \frac b 2 \rfloor^{rh(u)} \ge 2\lfloor \frac b 2 \rfloor^{rh(u)-1} = 2 \lfloor \frac b 2 \rfloor^{rh(u)-weight(u)}$.

\textbf{Inductive step.}
Suppose the claim holds before an update $U$.
We prove it holds after $U$.
Let $rh'(u)$ be the relaxed height of a node $u$ after $U$.

Suppose $U$ is Delete.
Then, each \iset\ remains the same, and every node has the same relaxed height before and after $U$.

Suppose $U$ is Insert.
Then, each \iset\ either gains one new key, or remains the same, and every node has the same relaxed height before and after $U$.

Suppose $U$ is Root-Replace.
Let $p$ be the old root, and $u$ be its only child.
If $u$ has \weight\ one before $U$, then $rh'(u) = rh(p)-1$.
Otherwise, $u$ has \weight\ zero before $U$, so $rh'(u) = rh(p)$.
Any keys associated with $p$ before $U$ are associated with $u$ after $U$, so the \iset\ of the root is the same before and after $U$.

Suppose $U$ is Root-Zero.
Let $r$ be the relaxed height of the root before $U$.
By the inductive hypothesis, the \iset\ of the root contains at least $2 \big\lfloor \frac b 2 \big\rfloor^{r}$ keys before $U$.
Moreover, $U$ does not change any \iset.
After $U$, the relaxed height of the root increases to $r+1$ because the \weight\ of the root changes from zero to one, so the \iset\ of the root contains at least $2 \big\lfloor \frac b 2 \big\rfloor^r = 2 \big\lfloor \frac b 2 \big\rfloor^{(r+1)-1} = 2 \big\lfloor \frac b 2 \big\rfloor^{rh(root)-weight(root)}$.

Suppose $U$ is Absorb.
Let $u$ be the child before $U$ and $p$ be its parent.
In this case, $u$ is removed by $U$, and all of its associated keys are instead associated with $p$.
The \iset, \weight\ and relaxed height of $p$ are all the same before and after $U$.

Suppose $U$ is Split.
Let $u$ be the child before $U$ and $p$ be its parent.
In this case, $U$ creates a new child, $v$, of $p$ and moves all of $p$'s pointers (except for its pointers to $u$ and $v$) into $u$ and $v$, so that $u$ and $v$ each contain at least $\lfloor \frac{b+1}{2} \rfloor \ge \frac b 2$ pointers.
Observe that $rh'(u) = rh'(v) = rh'(p) = rh(p)$.
Each pointer in $u$ or $v$ after $U$ points to a node with relaxed height $rh(p)-1$.
By the inductive hypothesis, the \iset\ of every such node contains at least $\lfloor \frac b 2 \rfloor^{rh(p)-1}$ keys.
Therefore, the \iset s of $u$ and $v$ each contain at least $\frac b 2 \lfloor \frac b 2 \rfloor^{rh(p)-1} \ge \lfloor \frac b 2 \rfloor^{rh(p)} = \lfloor \frac b 2 \rfloor^{rh'(u)} = \lfloor \frac b 2 \rfloor^{rh'(v)}$ keys, and the \iset\ of $p$ contains at least $\lfloor \frac b 2 \rfloor^{rh'(u)} + \lfloor \frac b 2 \rfloor^{rh'(v)} = 2 \lfloor \frac b 2 \rfloor^{rh'(p)}$ keys.

Suppose $U$ is Overflow.
Let $u$ be the leaf that is full.
In this case, $U$ creates a new leaf $r$ and an internal node $p$ with \weight\ zero and pointers to $u$ and $v$, and moves half of the keys from $u$ into $v$.
After $U$, the \iset\ of $p$ contains at least $b+1$ keys.
Since $u$ and $v$ are leaves, $rh(p) = 1$, so $b+1 \ge 2 \lfloor \frac b 2 \rfloor^{rh(p)}$.
The \iset s of $u$ and $v$ each contain at least $\frac b 2$ keys.
Since $rh(u) = rh(v) = 1$, $\frac b 2 \ge \lfloor \frac b 2 \rfloor^{rh(u)} = \lfloor \frac b 2 \rfloor^{rh(v)}$.

Suppose $U$ is Compress or One-Child.
Let $p$ be the upper node and $k$ be its degree.
Observe that $U$ does not change the weight or relaxed height of any node, and does not remove any key from the \iset\ of $p$.
After $U$, $p$ has $\lceil \frac c b \rceil$ children that evenly share $c$ pointers or keys.
Thus, each child contains at least $\lfloor \frac{c}{\lceil c/b \rceil} \rfloor \ge \lfloor \frac{c}{c/b+1} \rfloor = \lfloor \frac{cb}{c+b} \rfloor = \lfloor \frac{b}{1+b/c} \rfloor$ pointers or keys.
If $U$ is One-Child, then $c > kb-b$ and $k \ge 2$, so $c > b$ and $\lfloor \frac{b}{1+b/c} \rfloor > \lfloor \frac b 2 \rfloor$.
If $U$ is Compress, then two cases arise.
If $p$ has at least two children after $U$, then $\lceil \frac c b \rceil \ge 2$, so $c/b+1 \ge 2$ and $b/c \le 1$.
Therefore, each child of $p$ contains at least $\lfloor \frac{b}{1+b/c} \rfloor \ge \lfloor \frac b 2 \rfloor$ pointers or keys after $U$.
Otherwise, after $U$, the single child of $p$ contains all of the pointers and keys of the children that were removed, so its \iset\ is at least as large as it was before $U$.
The claim then follows immediately from the inductive hypothesis.
\qed
\end{proof}

\begin{cor}
Consider a \rbslack\ that results from performing a sequence of operations, $i$ of which are insertions, on a \bslack\ containing $n$ keys.
%Consider a \rbslack\ that results from performing a sequence of operations on a \bslack\ $T$, $i$ of which are insertions.
%Let $T$ be a \bslack\ that is transformed into a \rbslack\ by a sequence of operations. %Suppose a sequence of operations are performed on a \bslack\ $T$.
The relaxed height of the root, and, hence, any node in this \rbslack\ is at most $\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor + 1$.
\end{cor}

\begin{lem} \label{lem-upper-bound-on-splits}
After a sequence of operations, $i$ of which are insertions, on a \bslack\ containing $n$ keys, the total number of Absorb and Root-Zero updates that can be performed is at most $i$, and the number of Split updates that can be performed is at most $i (1+\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor)$.
\end{lem}
\begin{proof}
Absorb or Split is performed when a node has \weight\ zero.
Overflow is the only update that increases the number of zero \weight s in the tree, and at most $i$ Overflows occur, so there are at most $i$ nodes with \weight\ zero in the tree.
Absorb and Root-Zero each decrease the number of zero \weight s in the tree by one, so at most $i$ of these updates can be performed.
Root-Zero, Root-Replace, Absorb and Split are the only updates that can change the relaxed height of a node with \weight\ zero.
Root-Zero, Root-Replace and Absorb each change a zero \weight\ to one, and Split moves a zero \weight\ from a node with relaxed height $r$ to a node with relaxed height $r+1$.
%Split moves a zero \weight\ from a node with relaxed height $r$ to a node with relaxed height $r+1$.
%Split is the only update that moves a zero \weight, and no other update changes the relaxed height of a node with \weight\ zero.
Therefore, each zero \weight\ will remain at a node with the same relaxed height until it is moved by Split or changed to one by Root-Zero, Root-Replace or Absorb.
Since the relaxed height of any node in the tree is at most $\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor + 1$, each of the $i$ zero \weight s in the tree can be moved by Split at most $\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor + 1$ times.
\qed
\end{proof}

\begin{lem} \label{lem-amortized-rebalancing}
Let $T$ be a \rbslack\ of height $h$ that is obtained by performing any sequence of $i$ insertions and $d$ deletions on an initially empty \rbslack.
At most $2i(4+\frac 3 2 \big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor) + 2d/(b-1)$ rebalancing steps can be applied to~$T$.
\end{lem}
\begin{proof}
Let $c$ be the total degree of the children of a parent where Compress or One-Child is performed.
We first bound the number of One-Child updates that can be performed.
If a node has exactly one pointer, we say a \textit{pointer violation} occurs at that node.
One-Child is performed only when a pointer violation occurs at a child of the parent and $c > kb-b$.
Since $c > kb-b$ and $k \ge 2$, $c \ge b+1$, so the parent will have at least two children after One-Child.
Furthermore, each child of the parent will have degree at least $\lfloor b/2 \rfloor$.
Thus, One-Child removes every pointer violation at a child of the parent, and does not create any pointer violation.
Root-Replace removes a pointer violation at the root, decreasing the number of pointer violations in the tree by one.
However, Compress can \textit{increase} the number of pointer violations in the tree by one if $c \le b$.
No other update changes the number of pointer violations in the tree.
Therefore, the total number of One-Child and Root-Replace updates that can be performed is bounded above by the number of Compress updates.

We bound the number of Compress updates by studying the change in the total amount of slack in the tree that is caused by each type of update.
It is convenient to ignore the slack in any node with a zero \weight\ value, since Compress cannot affect any such node.
Compress redistributes a total of $c < kb-b$ pointers or keys from $k$ nodes to $\lceil c/b \rceil$ nodes.
Since $c \le kb-b = b(k-1)$, $\lceil c/b \rceil \le k-1$, Compress will remove at least one node from the tree.
Removing this node removes $b$ slack, and increases slack at the parent by one.
Thus, Compress reduces the total amount of slack in the tree by at least $b-1$ (and by even more, if more than one node is removed).
Split is applied precisely when the parent of a node with \weight\ value zero contains exactly $b$ pointers (and no slack).
Since the node with \weight\ value zero contains exactly two pointers, $b+1$ pointers are moved into the nodes with \weight\ value one in Figure~\ref{fig-updates}, so Split increases the total slack in the tree by exactly $b-1$.
By Lemma~\ref{lem-upper-bound-on-splits}, Split can be performed at most $i (1+\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor)$ times, so the total amount of slack created by Split is at most $i(1+\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor)(b-1)$.
It is easy to verify that Insert, Insert-Distribute and Absorb each decrease the total slack by one, and that Delete and Insert-Overflow increase the total slack by one and $2(b-1)$, respectively.
Thus, the total slack created by Delete and Insert-Overflow updates is $d + 2i(b-1)$, so the total slack in $T$ is at most $i(1+\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor)(b-1) + d + 2i(b-1) = i(b-1)(3+\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor) + d$.
Therefore, at most $i(3+\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor) + d/(b-1)$ Compress updates can occur.

By Lemma~\ref{lem-upper-bound-on-splits} at most $i$ Absorb and Root-Zero updates and $i (1+\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor)$ Split updates can occur.
Since the total number of Root-Replace and One-Child updates is at most the number of Compress updates, the number of Root-Replace, One-Child and Compress updates that can occur is at most $2i(3+\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor) + 2d/(b-1)$.
Therefore, at most $2i(3+\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor) + 2d/(b-1) + i + i (1+\big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor) = 2i(4+\frac 3 2 \big\lfloor \log_{\lfloor\frac{b}{2}\rfloor} \frac{n+i}{2} \big\rfloor) + 2d/(b-1)$ rebalancing steps can be applied to $T$.
\qed
\end{proof}

This result implies that the number of rebalancing steps needed to rebalance the tree after a sequence of deletions is amortized constant, and after a sequence of insertions is amortized logarithmic in the size of the tree the last time it was a \bslack, plus the number of insertions that have occurred since then. %, where $h$ is the height of the tree after all insertions.
%In Section~\ref{sec-analysis}, we prove that the height is logarithmic.
Section~\ref{sec-constant-rebalancing} explains how \bslack s can be modified to obtain amortized constant rebalancing by slightly increasing the amount of slack shared amongst the children of an internal node.

%\trevor{note to self: we should be able to get $O(b \cdot h(T))$ rebalancing updates from the previous lemma, and plug in the $h(T)$ later.}
%
%\trevor{Mention: by making a small change to the compress operation, we get amortized constant rebalancing. Explain in appendix.}

\section{\bslack s with Amortized Constant Rebalancing} \label{sec-constant-rebalancing}

The main challenge in achieving amortized constant rebalancing is ensuring that long sequences of Split and Compress operations occur infrequently.
Split can necessitate other Splits higher in the tree and many Compresses.
Compress can necessitate many other Compresses.
This makes Split and Compress particularly problematic.
%The other rebalancing steps do not lead to long sequences of rebalancing steps.

Split occurs only when an internal node is full.
If a Compress at an internal node leaves some slack in each of its children, 
then Splits will not immediately occur at the children.
With this in mind, we make some small modifications.
%to P\ref{prop-bslack-slack}, the definition of a slack violation and Compress.
P\ref{prop-bslack-slack} is replaced with P\ref{prop-bslack-slack}$'$, which says that, for each internal node $u$ of degree $k$, the total slack contained in the children of $u$ is at most $b+k-1$ (so the worst-case slack per node is only one greater than in a standard \bslack).
A slack violation then occurs at any internal node that violates P\ref{prop-bslack-slack}$'$.
The children of an internal node of degree $k$ where a slack violation occurs will have total degree less than $kb-(b+k-1)=(k-1)(b-1)$.
Thus, Compress is performed only at internal nodes whose children have total degree $c \le (k-1)(b-1)$, and One-Child is performed only at internal nodes whose children have total degree $c > (k-1)(b-1)$.
This threshold is chosen so that Compress is only performed when it can remove one node and still leave each child with one slack.
We then change Compress so that it evenly distributes the $c$ pointers or keys of its children amongst $\lceil \frac{c}{b-1} \rceil$ nodes, instead of $\lceil \frac{c}{b} \rceil$.
This way, each child is guaranteed to have at least one slack afterwards.

We prove that the number of rebalancing steps is amortized constant using the potential method. 
The potential of a node $u$, denoted $\phi(u)$, captures the intuition that
a node is bad when it contains too much slack, it is full, or it has \weight\ zero.
%it is bad when a node contains too much slack, and it is bad when a node is full or has \weight\ zero.
\begin{displaymath}
   \phi(u) = \left\{
     \begin{array}{ll}
       b-deg(u) & \mbox{if $deg(u) < b$ and $u$ has \weight\ one} \\
       b & \mbox{otherwise (i.e.,\ $deg(u) = b$ or $u$ has \weight\ zero)}
     \end{array}
   \right.
\end{displaymath}
The potential of a tree $T$, denoted $\Phi(T)$, is the sum of potentials of its nodes.


We now study how $\Phi(T)$ is changed by deletion, insertion, and each rebalancing step.
Let $u$ be a node with degree $k$. Recall that leaves never have \weight\ zero.

\textbf{Delete.}
If $u$ is full, then $\phi(u)$ changes from $b$ to $1$.
Otherwise, $\phi(u)$ changes from $b-k$ to $b-(k-1)$.
So, $\phi(u)$ increases by at most one.

\textbf{Insert.}
If the insertion fills $u$, then $\phi(u)$ changes from $1$ to $b$.
Otherwise, $\phi(u)$ changes from $b-k$ to $b-(k+1)$.
So, $\phi(u)$ increases by at most $b-1$.

\textbf{Overflow.}
A full node with potential $b$ turns into a node with \weight\ zero, which has potential $b$, and two nodes with \weight\ one that share a total of $b-1$ slack.
Thus, $b$ potential is replaced by $b+b-1=2b-1$ potential, which is an increase of $b-1$.

\textbf{Absorb.}
Let $u$ be the node with \weight\ zero. Its parent $\pi(u)$ has \weight\ one.
Beforehand, $u$ has degree two and $\pi(u)$ contains $j \leq b-1$ pointers, so is it not full.
%Let $v$ be the upper node and $u$ be the lower node.
%Since $u$ has \weight\ zero, it has degree two.
%Thus, $\pi(u)$ is not full before the Absorb.
Absorb decreases potential by $b$ by eliminating $u$.
It also moves a pointer from $u$ to $\pi(u)$.
%Let $j$ be the degree of $v$ before the Absorb.
If $j=b-1$, then $\phi(\pi(u))$ changes from 1 to $b$, increasing potential by $b-1$, for a net decrease of one.
Otherwise, $\phi(\pi(u))$ changes from $b-j$ to $b-(j-1)$, for a net decrease in potential of $b-1$.

\textbf{Split.}
Let $u$ be the node with \weight\ zero. Its parent $\pi(u)$ has \weight\ one, but it is full, so
it has potential $b$ behorehand. Afterwards, it has \weight\ zero, so its potential does not change.
%Let $v$ be the upper node and $u$ be the lower node.
Before the Split, $u$ has potential $b$, and it is split into two nodes, each of \weight\ one, that share a total of $b-1$ slack.
After the Split, the sum of their potentials is $b-1$.
Thus, the potential of the tree is decreased by one.

\textbf{Compress.}
%We would like to show that Compress decreases the total potential in the tree.
Let $u$ be a node with $k \geq 2$ children that have total degree at most $(k-1)(b-1)$.
%the upper node.
%Compress removes at least one node and distributes its keys to the remaining siblings.
%THIS IS NOT QUITE ACCURRATE
The modified version of Compress will leave at least one slack at each child of $u$, so the total potential of $u$'s children will be the total amount of slack they contain, which decreases by at least $b$, since
at least one of the children is removed.
Removing a child of $u$ also increases the slack at $u$ by one, which increases $\phi(u)$ by one (unless $u$ was full, in which case it decreases $\phi(u)$).
For each child of $u$ that is removed by Compress, $b$ slack is eliminated at at the children of $u$, and one slack is added at the parent.
Therefore, the total potential of the tree decreases by $b-1$ for each child removed by Compress.
Since at least one child is removed, the total potential of the tree decreases by at least $b-1$.

\textbf{One-Child.}
Since One-Child evenly distributes keys, it cannot create any more full nodes than existed beforehand.
It does not affect \weight s, and it does not remove any key or pointer.
So, One-Child does not affect the total potential of the tree.

Since $\Phi(T)$ is increased by one for Delete and $b-1$ for Insert (and Overflow), and no other operation increases it, after $i$ insertions and $d$ deletions, $\Phi(T) \le (b-1)i+d$.
We can use $\Phi(T)$ to bound the number of rebalancing steps that can be performed on $T$.
Let $C$, $A$, $S$, $R_0$, $R_r$ be the number of Compresses, Absorbs, Splits, Root-Zeros and Root-Replaces, respectively.
We immediately obtain $(b-1)C + A + S + 2(R_0 + R_r) \le \Phi(T) \le (b-1)i+d$.
Astute readers will notice that One-Child has not yet made an appearance.
By the same argument as in Lemma~\ref{lem-amortized-rebalancing}, the number of One-Childs is at most $C$.
Therefore, the number of rebalancing steps is constant per update.

In fact, we can achieve tighter bounds if we are more careful.
By the same argument as in Lemma~\ref{lem-upper-bound-on-splits}, $A + R_0 \le i$.
Additionally, the same argument used to show that the number of One-Childs is at most $C$ applies to Root-Replace, so $R_r \le C$.
Therefore, on average, there is at most one Absorb or Root-Zero per insertion, at most one Compress (and One-Child) and Root-Replace per insertion, and at most one Split per insertion.
Similarly, on average, there is at most one Absorb, Split, Root-Replace or Root-Zero per deletion, and at most one Compress (and One-Child) per $b-1$ deletions.

The increase in space complexity associated with these changes is very small.
Since the worst-case slack per node is only one greater than in a \bslack, the minimum average degree of this modified \bslack\ is at most one less than in a \bslack.
So, worst-case utilization changes from $\bar D/b$ to $(\bar D - 1)/b$, and space complexity changes from $2b(n-1)/(\bar D - 1) < 2b(n-1)/(b-3)$ to $2b(n-1)/((\bar D - 1) - 1) < 2b(n-1)/(b-4)$.


\section{Space Complexity of Competing Trees} \label{sec-competing}

In this section, we study the space complexity of some pathological families of B-trees, Overflow trees and H-trees.
The maximum degree of nodes is $b$, the block size is $2b$, and all trees are leaf-oriented.

\begin{itemize}
\item \textbf{B-tree.} The root has degree two, and all other nodes have degree $b/2$.
\item \textbf{Overflow tree.} The root has degree two, the internal nodes have degree $b/2$, and the leaves have degree $b-3$.
Overflow groups are chosen to be as large as possible, to minimize wasted space.
Specifically, for each parent $u$ of a leaf, $u$'s children are all in a single group, with one shared overflow node.
Thus, each overflow node is shared by $b/2$ leaves (which contain a total of $(b-3)(b/2) = b^2/2-3b/2$ keys).
\item \textbf{H-tree.} Parameters $\gamma$ and $\delta$ are chosen to be as large as possible, to minimize wasted space.
The root has degree two, the internal nodes have degree $\lceil b/\sqrt{2} \rceil$, and the leaves have degree $b-2$.
(H-trees are node-oriented, which inflates their space complexity on a system with only one block size.
%So, the H-trees considered here are leaf-oriented.
To actually achieve the space complexity values given in Figure~\ref{fig-spk}, one would have to design a leaf-oriented version of H-trees.) % A node-oriented H-tree would have significantly worse space complexity on a system with only one block size.)
\end{itemize}

We assume that a key and a pointer each occupy a single word in memory.
For each family, and each choice of maximum degree in $\{8,16,32\}$, we consider the minimum height tree from the family containing at least $10^6$ keys, and computed its space complexity.
Each tree contains between $10^6$ and $2 \times 10^6$ keys.
These space complexity values appear in Figure~\ref{fig-spk}, along with pessimistic upper bounds on the space complexity for any \bslack\ ($b \in \{8,16,32\}$) containing at least $50,000$ keys.
(The aforementioned upper bounds actually apply to \maxslack s, which allow the slack shared amongst the children of a node to be one greater than in a \bslack.)

The optimal space to store $n$ keys and pointers to associated data is $2n$.
H-trees, the closest competitor to \bslack s, use more than double the space beyond what is optimal.
If these trees were modified to implement a set instead of a dictionary (by eliminating data and allowing leaves to contain up to $2b$ keys), then the optimal space would become $n$, and it is expected that relative differences in space complexity between the trees would increase.

\renewcommand{\tabcolsep}{2mm}
\begin{figure}[tb]
\centering
\begin{tabular}{|c|ccccc|}
\hline
Max degree & B-tree & Overflow tree & H-tree & \bslack & Optimal \\
\hline
8  & $\ge 5.333n$ & $\ge 5.066n$ & $\ge 3.840n$ & $< 2.789n$ & $2.000n$ \\
16 & $\ge 4.571n$ & $\ge 3.120n$ & $\ge 2.685n$ & $< 2.301n$ & $2.000n$ \\
32 & $\ge 4.266n$ & $\ge 2.492n$ & $\ge 2.307n$ & $< 2.145n$ & $2.000n$ \\
\hline
\end{tabular}
%\begin{tabular}{|c|ccccc|}
%\hline
%Operation & B-tree & Overflow tree & H-tree & SDM-tree & \bslack \\
%\hline
%Insert & $\Theta(\log n)$ & $\Theta(\log n)$ & $\Theta(\log n)$ & $O((\log n)^{m-2})$ & amortized $O(\log n)$ \\
%Delete & $\Theta(\log n)$ & $\Theta(\log n)$ & $\Theta(\log n)$ & $O(n)$ & amortized $O(\log n)$ \\
%\hline
%\end{tabular}
\caption{
    Space complexity of example trees, and worst-case bound for \bslack s.
}
\label{fig-spk}
\end{figure}











\section{Experimental results} \label{sec-exp}

\textbf{[[[Mention that we do not have control over memory layout in Java, and we cannot embed arrays inside nodes, so nodes contain pointers to arrays of keys/values/pointers, rather than the arrays themselves. The space complexities quoted below are computed assuming that nodes contain the key/value/pointer arrays (not pointers to them). Thus, these space complexities are not directly achieved by the implementation. However, we still expect the space complexity of the Java implementation to be fairly good, since the pointers to arrays merely consume three extra words of memory per node. (Of course, space may also be lost to fragmentation caused by the memory manager, and a small amount is wasted by extra fields added to each node and array by the garbage collection system.)]]]}

The \bslack\ was implemented in Java, and several experiments were performed.
Randomized trials were performed with several $b$ values, simulated workloads, and tree sizes.
Each trial was divided into two phases.
In the first phase, a \bslack\ was created and initialized by inserting and deleting (with 50\% probability each) keys drawn uniformly randomly from $[0,size)$, until the tree stabilized, containing approximately $size/2$ keys.
In the second phase, one million random insertions and deletions were performed with some specified probabilities, and each rebalancing step was recorded.
We considered probabilities: 50\% insertion and 50\% deletion (50i-50d), 90\% insertion and 10\% deletion (90i-10d), and 10\% insertion and 90\% deletion (10i-90d).
At the end of each trial, average degree and space complexity were computed.

%For brevity, a 
A small selection of results are shown here.
For 50i-50d, $b=16$ and $size=2^{20}=$ 1,048,576, there were approximately 1.2 rebalancing steps per successful update, average degree was approximately 15.5, and space complexity was less than $2.209n$.
In fact, with $size=2^{12}=$ 4,096, average degree was approximately 15.4, and space complexity was less than $2.226n$, which is substantially better than the theoretical average degree lower bound of 12.7 and space complexity upper bound of $2.726n$.
This suggests that average case performance is quite good for \bslack s.
For 50i-50d, $b=32$, and $size=2^{20}$, there were approximately 1.1 rebalancing steps per successful update, average degree was approximately 31.5, and space complexity was less than $2.097n$.
For 10i-90d, $b=16$ and $size=2^{20}$, there was less than one rebalancing step per successful update.
Even with 90\% of updates being deletion, average degree remained the same, and space complexity was less than $2.213n$.
For 90i-10d, there were approximately 1.2 rebalancing steps per successful update.
These results suggest that little rebalancing is required for random updates on uniform keys.

It is also interesting to understand how many rebalancing steps are performed for the longest running updates.
So, we plotted a histogram for one trial with parameters 50i-50d, $b=16$ and $size=2^{20}=$ 1,048,576 in Figure~\ref{fig-histogram}.
(Results for other trials, values of $b$ and simulated workloads are similar.)
The $x$-axis shows the number of rebalancing steps that were performed by a single update, and the $y$-axis shows how many updates performed $x$ rebalancing steps.
The total number of successful insertions and deletions was 500,326, and the height of the tree was four when the trial finished.
The most rebalancing steps performed by an update was 18, and 99.9\% of successful updates performed less than ten rebalancing steps.

\begin{figure}
\hspace{-1mm}\includegraphics[scale=0.27]{figures/fig-histogram.png}
\vspace{-6mm}
\label{fig-histogram}
\caption{Histogram showing the frequency of updates that perform a certain number of rebalancing steps in a randomized trial.}
\end{figure}















\section{Implemention Issues for Rebalancing} \label{sec-cleanup-impl}

One way to implement rebalancing is to explicitly maintain a collection of pointers to internal nodes where rebalancing steps must be performed.
After an update creates a violation, a rebalancing step is performed to fix that violation.
Every time a rebalancing step creates a violation, a pointer to the node where the violation occurs (or its parent, as appropriate) is added to the collection.
An update does not terminate until it has emptied the queue and performed rebalancing steps to fix all violations in the tree.

The number of internal nodes is quite small compared to $n$ (close to $\frac{n}{(b-2)^2}$), so the worst-case collection size may be reasonable for some applications.
Since the amortized number of rebalancing steps per update is small, most updates will result in a small collection.
We recommend using a small, fixed-size queue implemented with a circular array, and switching to a more computationally expensive algorithm if the queue becomes full.
For instance, when a process tries to enqueue a pointer and the queue is full, it can simply discard that pointer, and continue the algorithm, recording the fact that the a pointer was discarded.
Eventually, after enough rebalancing steps are performed, the queue becomes empty, and the process can traverse the tree to find any outstanding violations, repopulating the queue, and continuing the algorithm.
Although this approach is very expensive once the queue becomes full, it will not significantly increase the average running time of updates if the queue rarely becomes full.
The experimental results in Section~\ref{sec-exp} indicate that this approach could be practical, even with a very small bound on queue size.













\section{Concurrent \bslack\ Implementation} \label{sec-concurrent}

A concurrent data structure is \textit{non-blocking} if, from any point in which there are 
data structure operations in
progress, some operation eventually completes.
This is true no matter how the steps of processes are scheduled by an adversarial
scheduler, who can even crash some, but not all, of the processes performing operations.
Thus, if processes take steps that access the data structure infinitely often, then,
infinitely often, some data structure operation completes.
In particular, a non-blocking data structure cannot use locks.

Brown, Ellen and Ruppert~\cite{paper2} provide a general technique for obtaining efficient,
provably correct, non-blocking
implementations of relaxed balanced trees in which each node has indegree at most one.
It consists of a template for writing update operations that atomically replace a node and
a connected subgraph of nodes reachable from it by a new connected subgraph, provided
both subgraphs have the same out-neighbourhood.
This includes all of the update operations for \bslack s.
They prove that each update operation invoked by a process either succeeds to update the shared data structure as desired or fails to affect it at all.
Furthermore, if updates following their template are invoked infinitely often,
then updates succeed infinitely often.
Localized updates to disjoint parts of the tree can proceed concurrently.
In addition, they prove that queries, such as searches, that start from the root and proceed 
down a path always give correct answers, no matter what updates are in progress or how their steps are interleaved.






















\section{Conclusion} \label{sec-conclusion}

\textbf{[[[Rewrite conclusion]]]}

We introduced \bslack s, which have excellent %average degree and
space complexity in the worst case, and amortized logarithmic updates.
The data structure is simple, requires only one block size, and is well suited for hardware implementation.

Modifying the definition of \bslack s so that the total slack shared amongst the children of each internal node of degree $k$ is at most $b+k-1$, instead of $b-1$, yields a data structure with amortized constant rebalancing (with small constants), and only a slight increase in space complexity.
Specifically, such a tree containing $n > b^3$ keys occupies at most $\frac{2b}{b-4}n$ words.
Details appear in the full version of the paper.

The recently introduced technique of Brown, Ellen and Ruppert~\cite{paper2} can be used to obtain a concurrent implementation of \rbslack s that tolerates process crashes and guarantees some process will always make progress.
In the resulting implementation, localized updates to disjoint parts of the tree can proceed concurrently, and searches can proceed without synchronizing with updates, which makes them extremely fast.
The implementation can be designed such that, in a quiescent state, when no updates are in progress, the data structure is a \bslack.

%Appendix~\ref{sec-constant-rebalancing} describes a small modification to \bslack s that yields a data structure with amortized constant rebalancing (with very small constants), and only a very slight increase in space complexity.
%Specifically, the minimum average degree of the modified data structure is only one less than the minimum average degree of \bslack s, so the worst-case space complexity is bounded above by $2b(n-1)/(b-3.4)$ for $n > b^3$.

%Appendix~\ref{sec-competing} describes pathological families of B-trees, Overflow trees and H-trees, and compares the space complexity of example trees in these families with the worst-case upper bound on the space complexity of a \bslack.
%By studying these families, we obtain lower bounds on the space complexity of these trees that are above the upper bound for \bslack s.

\bslack s have been implemented in Java, and code is freely available from \url{http://implementations.tbrown.pro}.
Experiments have been performed to validate the theoretical worst-case bounds, and to better understand the level of pessimism in them.
The results indicate that few rebalancing steps are performed in practice, and average degree is somewhat better than the already good worst-case bounds.
For instance, for $b=16$ and $b=32$, over a variety of simulated random workloads with tree sizes varying between $2^5=$~32 and $2^{20}=$~1,048,576 keys, there were at most 1.2 rebalancing steps per insertion or deletion, and average degrees for trees were approximately $b-0.5$, which is extremely close to optimal.
%For instance, for $b=16$ and $b=32$, average degrees for trees produced by random updates on uniformly random keys were approximately $b-0.5$, which is extremely close to optimal.

%Appendix~\ref{sec-cleanup-impl} discusses some implementation details related to rebalancing.



%Appendix~\ref{sec-exp} gives experimental evidence that \bslack s are practical.
%In particular, the results suggest that, for updates on uniformly random keys, few rebalancing steps are performed, and average degree and space complexity are significantly better than in the worst-case.
%
%\trevor{describe contents of appendix; maybe move experimental results into paper?}
%
%any open questions?
%
%future work? get bounds on space complexity for the modified \bslack\ with amortized constant rebalancing.

\subsubsection{Acknowledgments}

This work was dramatically improved by the insightful comments of my supervisor, Faith Ellen.













\bibliographystyle{abbrv}
\bibliography{bibliography}

\end{document}


==> chap-desc/listingStyle.tex <==
%!TEX root = paper.tex

%\usepackage{microtype}
%\usepackage[T1]{fontenc}
%\usepackage[scaled]{beramono}
%%\usepackage{subcaption}
%\newcommand\Small{\fontsize{7}{7}\selectfont}
%\newcommand*\LSTfont{\Small\ttfamily\SetTracking{encoding=*}{-60}\lsstyle}
%\newcommand{\trevorlater}[1]{\textcolor{trevcolor}{\textbf{[[[#1--Trevor]]]}}}
\newcommand{\trevorlater}[1]{}
\newcommand{\trevor}[1]{\textcolor{trevcolor}{\textbf{[[[#1--Trevor]]]}}}
\newcommand{\maya}[1]{\textcolor{blue}{\textbf{[[[#1--Maya]]]}}}

%\lstdefinestyle{customc}{
%    belowcaptionskip=1\baselineskip,
%    breaklines=true,
%    %frame=L,
%    xleftmargin=\parindent,
%    language=C,
%    showstringspaces=false,
%    basicstyle=\LSTfont, %\scriptsize\ttfamily,
%    keywordstyle=\bfseries\color{green!40!black},
%    commentstyle=\itshape\color{purple!40!black},
%    %identifierstyle=\color{blue},
%    stringstyle=\color{orange},
%    numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
%    numbersep=5pt,                   % how far the line-numbers are from the code
%    numberstyle=\tiny\color{black}, % the style that is used for the line-numbers
%    otherkeywords={\#define},
%    escapechar=@,
%    otherkeywords={bool,word},           % if you want to add more keywords to the set
%}

%\definecolor{mygreen}{rgb}{0,0.6,0}
%\definecolor{mygray}{rgb}{0.5,0.5,0.5}
%\definecolor{mymauve}{rgb}{0.58,0,0.82}
%
%\lstset{ %
%  basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
%  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
%  breaklines=true,                 % sets automatic line breaking
%  captionpos=b,                    % sets the caption-position to bottom
%  commentstyle=\color{mygreen},    % comment style
%  %deletekeywords={...},            % if you want to delete keywords from the given language
%  %escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
%  %extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
%  frame=trBL,	                   % adds a frame around the code
%  %frameround=fttt,  
%  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
%  keywordstyle=\color{blue},       % keyword style
%  %language=Octave,                 % the language of the code
%  %otherkeywords={*,...},           % if you want to add more keywords to the set
%  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
%  numbersep=7pt,                   % how far the line-numbers are from the code
%  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
%  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
%  %showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
%  %showstringspaces=false,          % underline spaces within strings only
%  showtabs=false,                  % show tabs within strings adding particular underscores
%  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
%  stringstyle=\color{mymauve},     % string literal style
%  tabsize=2,	                   % sets default tabsize to 2 spaces
%  %title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
%}

==> chap-desc/old-alg-detailed.tex <==

\begin{figure}[t]
	%    \vspace{-3mm}
	\lstinputlisting[frame=single,tabsize=2,firstnumber=auto,name=code,language=C, style=customc,firstline=2,lastline=6]{code.c}
	%\vspace{-5mm}
	\caption{User defined macros and data.}\label{code-transformation-user-definitions}
	%\vspace{-4mm}
\end{figure}

\begin{figure}[t]
	%\vspace{-3mm}
	\lstinputlisting[frame=single,tabsize=2,firstnumber=last,name=code,language=C, style=customc,firstline=9,lastline=31]{code.c}
	%\vspace{-5mm}
	\caption{Internal macros (used only by other macros).}\label{code-transformation-bit-manipulation}
	%   \vspace{-4mm}
\end{figure}

\begin{figure}[t]
	%\vspace{-4mm}
	\lstinputlisting[frame=single,tabsize=2,firstnumber=last,name=code,language=C, style=customc,firstline=34]{code.c}
	%\vspace{-5mm}
	\caption{User-invoked macros for the transformation.}\label{code-transformation-functions}
	%\vspace{-4mm}
\end{figure}


\newcommand*\NEWLSTfont{\ttfamily\SetTracking{encoding=*}{-60}\lsstyle}
\newcommand{\seqptr}{{\NEWLSTfont{seqptr}}}
\newcommand{\seqmutable}{\texttt{seqAndMutable}}

\fakeparagraph{Detailed description} 
Our transformation is presented as a set of C macros.
C macros are similar to functions, but are slightly different.
A function invocation involves creating a new stack frame, pushing function arguments onto that stack frame, executing the body of the function, and then returning a value.
However, each macro invocation is simply replaced by the body of the macro, and any references in the macro's body to the macro's arguments are replaced by the plain text of the arguments passed to the macro invocation.
For example, if a macro is defined by \texttt{\#define MACRO(a, b) (a = b)}, then a macro invocation \texttt{MACRO(x->field, y+1)} will be replaced by the text \texttt{(x->field = y+1)}.
%For example, suppose we define a macro \textit{MAX} as follows: \texttt{\#define MAX(x, y) (x < y ? x : y)}.
%Then, when a piece of code invokes \texttt{MAX(
%In other words, when a piece of code invokes a macro $MACRO(x, y, z)$, the compiler takes the body of the macro and replaces all references 
%before the code is even compiled, a \textit{macro preprocessor} takes the replaces the macro invocation with the body of the macro (where all references to the macro arguments.
% and their arguments are also 
%instead of 
%their arguments are passed as plain text, rather than 
%presented as a set of user definitions, a set of internal C-style macros, and 
%We present the code transformation in three parts. 

\fakeparagraph{User definitions}
Figure~\ref{code-transformation-user-definitions} contains algorithm specific definitions that must be provided before using the transformation.
Specifically, one must specify an upper bound on the number of concurrent threads, and an upper bound on the number of bits needed to represent all mutable fields of a descriptor.
One must then add a \textit{seqAndMutable} field to each descriptor type to contain a sequence number and any mutable fields.
One must also declare a descriptor array for each type of descriptor used by the original algorithm.
%(The descriptor arrays are declared by the user, since the descriptor types are not known to our transformation macros.)
Note that each descriptor in the descriptor arrays should be padded to avoid false sharing~\cite{Scott:1993} (ideally by rounding the size of a descriptor up to a multiple of the cache line size, adding at least two cache lines of empty padding, and aligning descriptors to a cache line boundary).
%These definitions include the number of threads and the number of bits required for mutable fields and the definitions of the descriptors array. The definition of the descriptor array is part of the user code since the type of the descriptor is unknown to our transformation. 

\fakeparagraph{Internal macros}
Figure~\ref{code-transformation-bit-manipulation} contains macros that are invoked only by other macros in our transformation.
%The second part contains the transformation internal functions.
These are convenience macros for encoding and manipulating bit-fields.

Recall that each sequence pointer is conceptually divided into bit fields that contain the sequence number, thread name and user bits (as shown in Figure~\ref{fig-seqptr}.
Each of these bit fields is defined by an offset and a bit-width.
The thread name is defined by \textit{SEQPTR\_OFFSET\_TID} and \textit{SEQPTR\_WIDTH\_TID} (the latter of which is user defined).
The user bits field is defined by \textit{SEQPTR\_OFFSET\_USER} and \textit{SEQPTR\_WIDTH\_USER}.
The sequence number is defined by \textit{OFFSET\_SEQ} and \textit{WIDTH\_SEQ}, and this definition is used both for sequence pointers, and for the sequence number stored in descriptors.

%Similarly
%These macros define offsets and width for several bit fields, such as the user bits, thread name, and sequence number subfields in a sequence pointer.
%They also include convenience macros for manipulating these bit fields.
%%These are bit definitions and manipulation macros, used by the transformation, for both the sequence pointers, denoted \seqptr, and the co-located sequence and mutable fields, denoted \seqmutable. These macros are presented in Figure~\ref{code-transformation-bit-manipulation}. 


%Each part of sequence pointer and the co-located sequence with mutable fields is described as a combination of width and offset. As mentioned before, some of these need to be defined by the user since they are implementation specific. After the user defined these widths, the width of the remaining parts are established in lines \ref{code-transformation-width-offset-begin}-\ref{code-transformation-width-offset-end}.

Next, we define several bit manipulation macros.
The first, MASK (line~\ref{code-transformation-mask}), creates a bit mask, given an offset and width.
The second, GET (line~\ref{code-transformation-get}), returns the contents of a bit-field within a word, given its offset and width.
For the sake of readability, we use these macros to define shortcuts for reading important bit-fields: a sequence number (from a sequence pointer or \textit{seqAndMutable} field of a descriptor), a thread name, and any user-defined bits (lines~\ref{code-transformation-gets-start}-\ref{code-transformation-gets-end}).
We also define SEQPTR\_GET\_PTR, which obtains a pointer to a descriptor from a sequence pointer and descriptor array (line~\ref{code-transformation-get-ptr}).
Finally, we provide DESC\_GET\_MUTABLE to retrieve the value of a mutable field embedded in a \textit{seqAndMutable} field.
The exact encoding of these mutable fields in the bits of the \textit{seqAndMutable} field is known only to the user, so the macro takes a mask and offset as arguments.
%Finally, we define SEQPTR\_GET\_PTR, a macro that given the descriptor array and the \seqptr{} returns the pointer to the array cell (actual pointer), line~\ref{code-transformation-get-ptr}.  

\fakeparagraph{User-invoked macros}
%\textbf{Figure~\ref{code-transformation-functions} contains user-invoked macros}.
%The third part of our code transformation includes the external ADT functions, this part is presented in Figure~\ref{code-transformation-functions}. These functions are defined as macros.  
Our transformation involves adding invocations of the macros in Figure~\ref{code-transformation-functions} (sometimes in place of other steps in the original algorithm).

Whenever a thread in the original algorithm would allocate a descriptor, it now invokes DESCRIPTOR\_NEW (line~\ref{code-transformation-desc-new}).
This macro takes a descriptor array, thread name, and initial value for all mutable fields (packed as it would be in a \textit{seqAndMutable} field) as arguments.
It locates the thread's descriptor in the descriptor array, modifies its \textit{seqAndMutable} field by incrementing its sequence number and initializing the mutable fields, and returns a pointer to this descriptor (technically, at line~\ref{code-transformation-desc-new-return}).
Finally, on x86/64, it is necessary to issue a memory barrier to ensure that the change to the descriptor's sequence number is visible to all threads before the thread that invokes DESCRIPTOR\_NEW begins initializing the descriptor.
%(This allows other threads to determine that their accesses to the descriptor should fail.)
%The macro DESCRIPTOR\_NEW (line~\ref{code-transformation-desc-new}) is used instead of calling the allocate function. This macro receives the variavble name of the descriptor array, the thread id and the initial value of the mutable fields. The macro returns a pointer to the array cell of the thread as well as incrementing the sequence number and initializing the mutable fields (recall that these fields are co-located with the sequence number). 

After invoking DESCRIPTOR\_NEW, the a thread can use the pointer it returns to initialize all immutable fields, as usual.
Once it finishes, it invokes DESC\_INITIALIZED (line~\ref{code-transformation-desc-init}).
This macro increments the descriptor's sequence number a second time (to an even number), indicating that initialization is complete.
Only after this can the thread publish a sequence pointer to this descriptor.
Thus, only even sequence numbers are published.
Between consecutive invocations of DESC\_NEW and DESC\_INITIALIZED on a descriptor $d$, any accesses to $d$ by other threads will fail.
This prevents threads from seeing an inconsistent view of a descriptor while it is being initialized.
After initialization, the thread can read immutable fields of its descriptor directly, but must perform all other accesses to the descriptor by invoking macros.
Furthermore, other threads can access this descriptor only by invoking macros.

Next, the thread invokes a macro SEQPTR\_NEW, which constructs a new sequence pointer to a descriptor, given a descriptor array and thread name.
%The thread then ``forgets'' its pointer to the descriptor.
Whenever the thread would install a pointer to the descriptor in the original algorithm, it now installs this sequence pointer.
%The value to publish is obtained using the SEQPTR\_NEW macro, line~\ref{code-transformation-seqptr-new}. The values passed to this macro are the descriptors array, tid and the user bits. This function obtains the current sequence number using the descriptor array and tid, and then creates the \seqptr{} by concatinating the sequence, tid and the user bits.   

Reads of immutable fields in the original algorithm can be transformed in two different ways.
A single field can be read by calling DESC\_READ\_IMMUTABLE (line~\ref{code-transformation-read-immutable}).
This takes the name of a temporary variable, a sequence pointer, a descriptor array, and a field name, as its arguments.
The macro uses the descriptor array and sequence pointer to locate the appropriate descriptor, then reads the desired field, and validates the read by comparing the sequence numbers in the sequence pointer and descriptor.
The result of this validation is stored in the temporary variable, which the invoking thread uses to determine whether its read succeeded (true) or failed (false).
%The sequence pointer is passed to this macro and is used to validate the read. The result of the validation is saved in a specified location. To ensure consistency the thread must check that it is true before using the value.
This validation cost is incurred for every read performed this way.
%Using this macro will result in validation for every read. 
If the thread will read most or all of the immutable fields of the descriptor, then DESC\_SNAPSHOT offers a more efficient option.
This macro copies the entire descriptor and then performs a single validation check.
If the validation succeeds then the thread can read immutable fields freely from the snapshot.
%If the thread is likely to read all the immutable fields of the descriptor DESC\_SNAPSHOT can also be used, line~\ref{code-transformation-snapshot}. This macro copies the entire descriptor and then validate it. If the validation succeeds then the thread can read immutable fields from the created copy, without any additional validation. 

%In our transformation, the mutable fields are a set of bits that are part of \seqmutable word. The user, however, has the knowlage of which bits belong to wich mutable field. Therefore, every operation on the mutable fields receives a mask and offset values needed to extract the desired field out of the \seqmutable{} word. 

Mutable fields are always read from the descriptor using DESC\_READ\_MUTABLE (line~\ref{code-transformation-read-mutable}), since they may change repeatedly throughout an operation, so they cannot simply be read from a static snapshot.
%are co-located with the sequence number.
The algorithm for reading them is similar to DESC\_READ\_IMMUTABLE. %, but the validation is slightly different. 

Mutable fields can be modified using two different macros, DESC\_WRITE\_MUTABLE and DESC\_CAS\_MUTABLE (lines~\ref{code-transformation-write-mutable} and~\ref{code-transformation-cas-mutable}).
These macros use CAS to ensure that fields are modified only if the sequence number has not changed.
These CAS steps might fail due to a concurrent write (to the same field or a different field) or due to a change to the sequence number.

In DESC\_WRITE\_MUTABLE, failed CAS steps are retried as long as the sequence number has not changed, and the field does not contain the desired value.
(Thus, it will terminate only if the descriptor is reused, or a CAS has successfully stored the value, mimicking a write in the original algorithm.)
\begin{fullver}
	The macro sets its first argument \textit{result} to true if it succeeds, and false if it failed (because the descriptor was reused).~
\end{fullver}
\begin{shortver}
	The macro sets its first argument \textit{result} to true if it succeeds, and false if it failed.~
\end{shortver}

In DESC\_CAS\_MUTABLE, failed CAS steps are retried as long as the sequence number has not changed, and the field contains the expected value.
The macro CAS\_MUTABLE sets its first argument \textit{result} to true if it changes the field, false if the field did not contain the expected value, and \textit{FAILED} if it failed because the descriptor was reused.


\fakeparagraph{Problems with unbounded sequence numbers}
%see my paper for the details
%
Unbounded sequence numbers can cause errors if used indiscriminately.
In our transformation, there are two potential issues.

The first issue arises when threads can sleep for an extremely long time.
Suppose a thread $p$ reads a pointer to a descriptor with version $v$ that was created by thread $q$, and reads one field of the descriptor.
Then, $p$ sleeps for a very long time, until the sequence number in $q$'s descriptor wraps around to the exact same value $v$.
Finally, $p$ wakes up and reads a second field of the descriptor.
The second read by $p$ is successful, because $q$'s descriptor contains version $v$.
However, $p$'s view of $q$'s descriptor is inconsistent, since its second read was performed after $q$ has reused its descriptor many times.
Consequently, $p$ can perform arbitrary steps that are not possible in the original algorithm.
If the sequence number is very large, then the probability of a thread sleeping until the sequence number wraps around to the exact same value is infinitesimal.
In the following, we assume the sequence number is sufficiently large so that \textit{threads always see a consistent view of each descriptor they access}.
\begin{fullver}
	(We perform experiments to study how likely this is with different sequence number sizes in Section~\ref{sec-exp-wraparound}.)
\end{fullver}

The second issue arises if descriptor pointers can remain in the data structure long after the operations that created them have completed.
Suppose a thread $p$ installs a pointer to a descriptor with version $v$ into the data structure in a memory location $addr$ at time $t$.
Moreover, suppose $p$ performs sufficiently many operations for its descriptor to once again have version $v$ at time $t' > t$, and that $addr$ is not modified between $t$ and $t'$.
Then, another thread $q$ can read $addr$ at time $t'$, and see a pointer to $p$'s descriptor, at which point it tries to read a field of $p$'s descriptor, and succeeds since the version is $v$.
In this case, $q$ is accessing $p$'s \textit{current} descriptor version through a pointer to one of $p$'s \textit{old} descriptor versions.
(Note, however, that $q$ will see a \textit{consistent} view of $p$'s current descriptor version.)
Consequently, $q$ may decide to help $p$'s current operation.
Although this helping step would not have happened in the original algorithm, performing additional helping does not affect correctness or progress.


\fakeparagraph{Correctness and progress}
%
Due to lack of space, we omit formal proofs of correctness and progress.
Here, we simply give some intuition as to why the transformation is correct.
The transformation only affects accesses to fields of descriptors.
All threads see consistent views of the descriptors they access, as in the original algorithm. %so threads performing \textit{Help} only take actions they could have taken in the original algorithm
However, after the transformation, some accesses may now fail, where they would not before.
If these failed accesses occur only in invocations of \textit{Help}, then they simply cause threads to stop helping (and helping is no longer necessary).

Suppose some failed accesses occur outside of invocations of \textit{Help}.
Then, to apply our transformation, one must identify what actions a thread should take after each failed access, and make ad-hoc arguments that these actions preserve correctness.
As we will see in Section~\ref{sec-kcas}, this can be as simple as identifying a specific value that a failed read should ``return'' such that a thread takes precisely the same actions it would take if the version of the descriptor that it tried to access still existed (i.e., the same actions the thread would take in the original wasteful algorithm).
%For some algorithms One way of doing this is to identify 
%ad-hoc arguments must be 

Regarding progress, every step added by our transformation is wait-free, except for \textit{DESC\_WRITE\_MUTABLE} and \textit{DESC\_CAS\_MUTABLE}, which contain unbounded loops.
A thread can continue performing iterations of these loops only as long as other threads helping the \textit{same operation attempt} change mutable fields in the descriptor. %perform writes or \textit{successful} CAS steps on the same word, in each iteration.
Thus, if each operation attempt in the original algorithm completes after a bounded number of state changes, progress is guaranteed.

==> chap-template/ravl/rotations-style.tex <==
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}

\usepackage{anysize}
\marginsize{0cm}{0cm}{-1cm}{0cm}
%\usepackage{geometry}
\usepackage{pgf}
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,snakes,automata,backgrounds,petri}

\tikzstyle{tri} = [regular polygon,regular polygon sides=3,draw=black!80,fill=blue!13,minimum size=16mm]
\tikzstyle{dashed square} = [rectangle,dotted,draw=black!80,minimum size=5mm]
\tikzstyle{regularnode} = [circle,draw=black!80,fill=blue!13,minimum size=5mm]
\tikzstyle{leafnode} = [rectangle,draw=black!80,fill=blue!13,minimum size=5mm]
\tikzstyle{ghost square} = [rectangle,draw=black!35,fill=blue!5,minimum size=5mm]
\tikzstyle{ghost path} = [draw=black!35,thick,-]
\tikzstyle{place} = [circle,thick,draw=blue!80,fill=blue!13,minimum size=7mm]
\tikzstyle{red square} = [square,draw=black!80,fill=red!13]
\tikzstyle{red place} = [place,draw=red!75,fill=red!20]
\tikzstyle{green square} = [square,draw=black!80,fill=green!13]
\tikzstyle{invisiplace} = [minimum size=6mm]
\tikzstyle{every path} = [draw=black!80,thick,-]
\tikzstyle{soft path} = [draw=gray!80,-]
\tikzstyle{big path} = [draw=blue!50,-,double]
\tikzstyle{every label} = [black!70]
\tikzstyle{blacklabel} = [black]

